Global Unifying Intrinsic Calibration for Spinning and Solid-State LiDARs

Sensor calibration, which can be intrinsic or extrinsic, is an essential step to achieve the measurement accuracy required for modern perception and navigation systems deployed on autonomous robots. To date, intrinsic calibration models for spinning LiDARs have been based on hypothesized based on their physical mechanisms, resulting in anywhere from three to ten parameters to be estimated from data, while no phenomenological models have yet been proposed for solid-state LiDARs. Instead of going down that road, we propose to abstract away from the physics of a LiDAR type (spinning vs solid-state, for example), and focus on the spatial geometry of the point cloud generated by the sensor. By modeling the calibration parameters as an element of a special matrix Lie Group, we achieve a unifying view of calibration for different types of LiDARs. We further prove mathematically that the proposed model is well-constrained (has a unique answer) given four appropriately orientated targets. The proof provides a guideline for target positioning in the form of a tetrahedron. Moreover, an existing Semidefinite programming global solver for SE(3) can be modified to compute efficiently the optimal calibration parameters. For solid state LiDARs, we illustrate how the method works in simulation. For spinning LiDARs, we show with experimental data that the proposed matrix Lie Group model performs equally well as physics-based models in terms of reducing the P2P distance, while being more robust to noise.

==> AutomaticCalibrationSystem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Automatic Calibration System}
\label{sec:AutomaticCalibrationSystem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Target-based \lc extrinsic calibration methods often suffer from manual target
extraction and feature association. The only manual process in our previous software
release \cite{huang2019improvements}, determining the image corners, has now been
made automatic. Because experimentally comparing and validating the intrinsic
calibration methods of Sec.~\ref{sec:IntrinsicCalibration} and~\ref{sec:Baseline}
would require significant data collection, we decided to create a fully automatic
pipeline for both intrinsic and extrinsic calibration, as shown in
Fig~\ref{fig:AutomaticPipeline}. We demonstrate the capability of this pipeline in
the experimental section by collecting a significant amount of data allowing us to
check the quality of the calibration of our sensor suite (a \lc pair) at different
distances; see Sec.~\ref{sec:EXPExtrinsicCalibration}.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{graphics/pipeline2.png}
    \caption{A system diagram for
        automatic intrinsic and extrinsic calibration. The top shows the front-end of
        the pipeline. Its input is raw camera and \lidar data, which are subsequently
        synchronized. The \atag and \lidart packages are used to extract the target
        information, which is then examined to remove outliers and ensure that
        targets are still properly synchronized. Each run of the front-end saves all
        related information into a ROS bagfile, which can then be sent to the
        back-end for further processing. The back-end takes in (possibly many) ROS
        bagfiles and does the following: (i) refines the image corners; and (ii)
        extracts vertices of the \lidar targets. The correspondences are established
        between corners and vertices and an extrinsic transformation is determined
        PnP as in \cite{lepetit2009epnp}. For intrinsic calibration, the resulting vertices of
        the \lidar targets are used to extract normal vectors and a point on the
        plane. The calibration parameters are determined to minimize the P2P distance
        from the plane to the target points provided by the \lidart package.} 
\label{fig:AutomaticPipeline}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Front-End}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Fiducial markers are widely used in vision-based perception tasks because they can
be easily identified and automatically extracted from the background.  Inspired by \atagsN \cite{olson2011apriltag, wang2016apriltag,
krogiusflexible}, we introduced a similar concept for \lidar point clouds,
called a LiDARTag, consisting of a payload and a pattern that
makes each marker uniquely distinguishable and identifiable in real-time by both a
\lidar and a camera 
\cite{huang2019lidartag}. An open-source package for processing \lidarts is available
\cite{githubFileLiDARTag}, while \atagN3 is available as a ROS package
\cite{githubFileAprilTagROS}. 

As \lidar and camera data streams arrive, they are synchronized, examined for
fiducial markers, and checked for false positives. For \lc extrinsic calibration, we use target
vertices and image corners as features. The relevant data (images, AprilTag corners, points on
\lidartsN) are saved as ROS bagfiles for processing in MATLAB. Technical details and software are
available at~\cite{githubFileAutoCalibration}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Back-End}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The back-end begins by estimating the \lidart vertices, which, due to sparsity of the \lidar point cloud, are not directly observable. We use the method developed in
\cite[Sec.~II]{huang2019improvements} to determine the vertices of a diamond-shaped target. A rigid-body transformation is determined that ``best fits'' the target's \lidar points to the target's known geometry. Best fit is defined in an $L_1$ sense. 


From the vertices, the target normal $\n[t]$ and point on the target, $\p[0,t]$, can
be easily determined for evaluating the P2P cost function \eqref{eq:OptSolution} for intrinsic calibration, while the vertices in combination with the camera corners are used to determine the extrinsic calibration via a PnP problem. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\columnwidth, trim={0.05cm 0cm 0cm 1cm},clip] {graphics/reference_frame2.png}
%     \caption{\bh{Notation}Target reference frame and real point cloud data.
%         The dotted blue square is the reference target; its vertices are denoted
%         $\{\bar{X}_i\}_{i=1}^4$.} 
% \label{fig:IdealFrame}
% \end{figure}

% \begin{figure}[t]%
% \centering
% \subfloat[]{%
% \label{fig:IdealFrame}%
% \includegraphics[width=0.45\columnwidth, trim={0.05cm 0cm 0cm 1cm},clip] {graphics/reference_frame2.png}}~
% \subfloat[]{%
% \label{fig:CannyLineFitted}%
% \includegraphics[width=0.48\columnwidth, trim={3.5cm 12.6cm 3cm 10cm},clip]{CannyLineFitted.png}}\\
% \subfloat[]{%
% \label{fig:CalibrationResults}%
% \includegraphics[width=0.45\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test6_3.png}}~
% \hspace{2pt}%
% \subfloat[]{%
% \label{fig:CannyLineFitted}%
% \includegraphics[width=0.5\columnwidth, trim={2cm 1.7cm 2cm 0.7cm},clip]{test6_3.png}}
% \caption[]{\bh{Notation, not much space, may remove
% later}\subref{fig:IdealFrame}Target reference frame and real point cloud data.
% The dotted blue square is the reference target; its vertices are denoted
% $\{\bar{X}_i\}_{i=1}^4$.\subref{fig:CannyLineFitted} shows the result of edge
% detection. }% 
% \label{fig:ImageEdgeDetection}%
% \squeezeup
% \end{figure}


 The corners obtained from the \atag package are automatically refined using a process detailed in \cite[Sec.V-C]{huang2019improvements}. Given the camera corners, denoted ($\{ Y_i\}_{i=1}^4$), and \lidar vertices, denoted $\{ X_i\}_{i=1}^4$, we use the vertical and horizontal positions in their own coordinates to sort them and establish the correspondences.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Intrinsic and Extrinsic Calibration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:InExCalibration}
For extrinsic calibration, the rigid body transformation between \lidar to camera is found by solving a Perspective-n-Point (PnP) problem as in \cite{lepetit2009epnp}, namely 
\begin{equation} 
    \label{eq:ConceptualProblem} (\R[L][C*], \t[L][C*])= \mathrm{arg}
    \min_{(\R,\t)}{\mathrm{dist}(P(\R X_i + \t),Y_i)}, 
\end{equation} 
where $X_i$ are coordinates of the \lidar vertices, $Y_i$ are the
coordinates of the camera corners, and $P$ is the standard 3D$\to$2D camera ``projection map'', based in its intrinsic parameters. Furthermore, $\R[L][C],\t[L][C]$ is the \lidarN-frame to camera-frame rigid body transformation, and $\mathrm{dist}$ is a distance or error
measure (typically $L_2$). For example results, see~\cite{huang2019improvements}.

With the method in \cite{huang2019improvements}, the target vertices are automatically co-planar and hence uniquely define a unit normal vector and a
point on the target. The P2P distance is minimized for each of the three calibration
models, \BL1, \BL2, and $\Sim(3)$, for a collection of targets, yielding $\alpha^*$
(for \BL1 and \BL2) and  $\H[*]$ for $\Sim(3)$.

For experimental data, the process of intrinsic calibration involves iterating the estimation of the
target vertices and the parameters in the \lidar model until a given stopping
criterion is met. Here, we stopped when the maximum change $\delta_m$ over the set of target vertices was less
than $1e-5$.

\begin{algorithmic}
\While{$\delta_m>10^{-5}$} 
\State \textbf{Step 1:} Re-estimate the target vertices $\{ X_i\}_{i=1}^4$
after applying the current intrinsic calibration parameters to the point
cloud. This gives updated values for the target normals and points on the
targets.
\State \noindent \textbf{Step 2:} Using the updated target vertices, re-estimate the intrinsic calibration parameters for the three calibration models.
\EndWhile
\end{algorithmic}
For simulation data, no iteration is required as the target information is known from ``ground truth''.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\subsection{System Overview}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \subsection{Sensor Synchronization and Feature Extraction}
% Due to the \lidar and camera data arriving at different rates, they have to be
% properly synchronized, especially, if the calibration scene is not static. Because
% the camera frames are roughly at 30 Hz and \lidar packets are at 10 Hz, the
% \textit{ApproximateTime} policy in Robot Operating System (ROS) can be used for
% synchronization ~\cite{quigley2009ros}. The synchronized data 
% are indexed and sent to appropriate packages for feature extraction.
% 
% Fiducial markers are widely used in navigation as well as
% vision-based simultaneous localization and mapping (SLAM). They often consist
% of a payload, a pattern that makes each marker uniquely distinguishable.
% Therefore, as an aid in the automatic identification of targets in
% camera and \lidar data, we build and use fiducial markers that can be identified by
% both a \lidar and a camera.  
% 
% 
% \subsubsection{camera targets}
% Images containing calibration targets are processed using the latest \atag3
% package~\bh{cite \atag1, \atag2, \atag3, Github}. The package is written in C++
% on the ROS platform and provides the (inner) corners of the fiducail marker and the
% corresponding ID. The target vertices, however, are the outer corners as shown in
% Fig~\bh{InnerOuterCorners}. Given the homography matrix and the intrinsic parameters of the
% camera, the outer corners can be determined with simple linear interpolation.
% For more detail, see~\bh{\atag1}
% 
% 
% \subsubsection{\lidar targets}
% Point clouds containing the calibration targets are sent to \lidart
% package\bh{cite}. \lidart is a type of fiducial marker that can be detected
% n real-time from \lidar point clouds, called \lidartsN.
% The released
% version of \lidart provides the points on the target and tag size associated with the target. The
% target points are then post-processed by an $L_1$-inspired norm to determine the vertices;
% see~\ref{sec:LiDARVertices} and \bh{cite}.
% 
% \begin{remark}
% don't care poses
% \end{remark}
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Target Association}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Due to false positive from detection algorithms, further examination of the extracted
% features is crucial. As mentioned, we have indexed the synchronized data and they are
% used as a tracking id. We have three messages to associate: images, \atags and
% \lidartsN. Each of them has its own queue and because images are raw measurement, we
% ensure the indices of the two types of detection are the same as the image's index,
% before publishing. We also create a global sequence queue to track the
% candidate index to publish. ~\bh{working on...}
% 
% % Whenever a new message arrives, the frame index of this message will pushed to
% % its own queue and the global sequence queue if it is in order. 
% % When the front of three message queues have the same frame index, we shall group them
% % together and publish.
% % 
% % Lastly, the detection messages with the same index are grouped as a new paired message. 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Finding LiDAR Corners and Corners Association}
% \label{sec:LiDARVertices}
% \label{sec:CornerAssociation}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% At this stage, extracted features (\atag corners and \lidart points) have been
% properly synchronized and cautiously examined. An $L_1$-inspired norm is applied to
% estimate non-directly observable \lidart vertices. Given Let $\pc := \{X_i\}_{i=1}^{M}$
% be the collection of 3D points on the \lidar target, where $M$ is the number of
% points. For $a \ge 0$ and $\lambda \in \real$, the $L_1$-inspired cost is defined as 
% \begin{equation}
%     \label{eq:L1cost}
%     c(\lambda,a):=\begin{cases} 
%     \min\{ |\lambda-a|, |\lambda + a| \} & \text{if}~|\lambda| >a \\
%     0 & \text{otherwise}
%     \end{cases},
% \end{equation}
% and the total cost is define as 
% \begin{equation}
% 	\label{eq:JKHcost}
%     C(H_T^L(\pc)) :=\sum_{i=1}^{M} c(\tilde{x}_i,\epsilon) +
%     c(\tilde{y}_i,d/2) +  c(\tilde{z}_i,d/2),
% \end{equation}
% where $\epsilon \ge 0$ is a tuning parameter to account for uncertainty in the depth
% measurement of the planar target. For more detail about this method and target
% placement for extrinsic calibration, see~\bh{cite}.
% 
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Extrinsic Calibration}
% \label{sec:ExtrinsicCalibration}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> ExperimentTablesOld.tex <==
% \begin{table}[]
% \caption{3-parameter perturbation model $(\N[1])$ for a spinning \lidar in the simulator}
% \label{tab:N2}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% N1 & scene1 & scene2 & scene3 & scene4 & scene5 & scene6 \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline1 & 0.036998 & 0.037076 & 0.034804 & 0.032165 & 0.017921 & 0.028471 \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline2 & 0.16108 & 0.15412 & 0.15745 & 0.035424 & 0.023221 & 0.023275 \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.020421} & \textbf{0.028072} & \textbf{0.013583} & \textbf{0.010428} & \textbf{0.0016329} & \textbf{0.0010792} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \caption{6-parameter perturbation model $(\N[2])$ for a spinning \lidar in the simulator}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% N2 & scene1(8) & scene2(9) & scene3(10) & scene4(25) & scene5(6) & scene6(7) \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline1 & 0.024689 & 0.025205 & 0.027227 & 0.021967 & 0.010316 & 0.012955 \\ \hline
% \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.14897 & 0.14993 & 0.14192 & 0.033905 & 0.012305 & 0.0086185 \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.015302} & \textbf{0.018722} & \textbf{0.012405} & \textbf{0.01152} & \textbf{0.003471} & \textbf{0.00076376} \\ \hline
% \end{tabular}
% \end{table}

% % \jwg{In Table~ref{tab:N3} scene 5, we are marked as winning but we lose}
% % \bh{I noticed, I am going to ask Chenxi later.}

% \begin{table}[]
% \caption{Induce $\Sim(3)$ noise model $(\N[3])$ for a spinning \lidar in the simulator.}
% \label{tab:N3}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% N3 & scene1(8) & scene2(9) & scene3(10) & scene4(25) & scene5(6) & scene6(7) \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline1 & 0.037758 & 0.037428 & 0.038231 & 0.033412 & 0.023682 & 0.031802 \\ \hline
% \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.16082 & 0.15571 & 0.15756 & 0.04164 & 0.022272 & 0.024862 \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.02297} & \textbf{0.025774} & \textbf{0.012842} & \textbf{0.013986} & \textbf{0.0053697} & \textbf{0.00010772} \\ \hline
% \end{tabular}
% \end{table}


% \begin{table*}[]
% \caption{Induce 3-parameter perturbation model $(\N[1])$,  6-parameter perturbation model $(\N[2])$, and $\Sim(3)$ noise model $(\N[3])$ for a spinning \lidar in the simulator.}
% \label{tab:N3}
% \center
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% Noise Model & Methods & \cellcolor[HTML]{C0C0C0}scene 1 & \cellcolor[HTML]{C0C0C0}scene 2 & \cellcolor[HTML]{C0C0C0}scene 3 & \cellcolor[HTML]{C0C0C0}scene 4 & \cellcolor[HTML]{C0C0C0}scene 5 & \cellcolor[HTML]{C0C0C0}scene 6 \\ \hline
% \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline1 & 0.036998 & 0.037076 & 0.034804 & 0.032165 & 0.017921 & 0.028471 \\ \cline{2-8} 
% \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.16108 & 0.15412 & 0.15745 & 0.035424 & 0.023221 & 0.023275 \\ \cline{2-8} 
% \multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}N1} & \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.020421} & \textbf{0.028072} & \textbf{0.013583} & \textbf{0.010428} & \textbf{0.0016329} & \textbf{0.0010792} \\ \hline
% \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline1 & 0.024689 & 0.025205 & 0.027227 & 0.021967 & 0.010316 & 0.012955 \\ \cline{2-8} 
% \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.14897 & 0.14993 & 0.14192 & 0.033905 & 0.012305 & 0.0086185 \\ \cline{2-8} 
% \multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}N2} & \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.015302} & \textbf{0.018722} & \textbf{0.012405} & \textbf{0.01152} & \textbf{0.003471} & \textbf{0.00076376} \\ \hline
% \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline1 & 0.037758 & 0.037428 & 0.038231 & 0.033412 & 0.023682 & 0.031802 \\ \cline{2-8} 
% \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.16082 & 0.15571 & 0.15756 & 0.04164 & 0.022272 & 0.024862 \\ \cline{2-8} 
% \multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}N3} & \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.02297} & \textbf{0.025774} & \textbf{0.012842} & \textbf{0.013986} & \textbf{0.0053697} & \textbf{0.00010772} \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\caption{Geometric uncertainty of a \sslidar by assuming the plane of the wafer is slightly warped.}
\label{tab:sslidar}
\center
\resizebox{\columnwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{C0C0C0}}c |c|c|c|}
\hline
Solid-State LiDAR & \cellcolor[HTML]{C0C0C0}Before Calibration & \cellcolor[HTML]{C0C0C0}After Calibration & \cellcolor[HTML]{C0C0C0}Improvement \\ \hline
Training results & 0.3315 & 0.0029 & 99.12 \% \\ \hline
Validation Scene1 & 0.2659 & 0.0197 & 92.59 \% \\ \hline
Validation Scene2 & 0.3193 & 0.0323 & 89.89 \% \\ \hline
Validation Scene3 & 0.2958 & 0.0202 & 93.16 \% \\ \hline
\end{tabular}
}
\end{table}



% \begin{table}[t]
% \caption{\bh{CHANGE. This is an old table using all 39 targets.} Experimental results of the automatic intrinsic calibration with targets arranged to avoid the degeneracies indicated in Prop.~\ref{thm:HopefullyTrue}.}
% \center
% \label{tab:RealExp}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
%  & Baseline1 & Baseline2 & Our Method \\ \hline
% \cellcolor[HTML]{C0C0C0}Validation Results & 0.0068 & 0.0082 & \textbf{0.0052} \\ \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[]
\caption{Experiments data collected using different numbers of targets in the calibration scene.}
\label{tab:RealExp}
\center
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
{\color[HTML]{000000} No.Tags} & 4 & 8 & 12 & 24 \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Baseline1} & \textbf{0.0064} & \textbf{0.0066} & 0.0066 & 0.0068 \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Baseline2} & 0.0146 & 0.0103 & 0.0083 & 0.0082 \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Our Method} & {\color[HTML]{000000} 0.0201} & {\color[HTML]{000000} 0.0084} & {\color[HTML]{000000} \textbf{0.0062}} & {\color[HTML]{000000} \textbf{0.0052}} \\ \hline
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% previous
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \caption{N2V13-Validation}
% \label{tab:N2V13}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% N2V13 & scene1(8) & scene2(9) & scene3(10) & scene4(11) & scene5(12) & scene6(6) & scene7(7) & scene8(14) \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline1 & 0.033529 & 0.0336 & 0.031541 & 0.033631 & 0.033397 & 0.029149 & 0.025802 & 0.033112 \\ \hline
% \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.14598 & 0.13967 & 0.14269 & 0.13876 & 0.034157 & 0.032103 & 0.021093 & 0.034269 \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.018507} & \textbf{0.025441} & \textbf{0.01231} & \textbf{0.011537} & \textbf{0.010229} & \textbf{0.00945} & \textbf{0.00097798} & \textbf{0.0014979} \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \caption{N3V13-Validation}
% \label{tab:N3V13}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% N3V13 & scene1(8) & scene2(9) & scene3(10) & scene4(11) & scene5(12) & scene6(6) & scene7(7) & scene8(14) \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline1 & 0.022374 & 0.022842 & 0.024675 & 0.023045 & 0.022249 & 0.019907 & 0.017763 & 0.01174 \\ \hline
% \cellcolor[HTML]{C0C0C0}BaseLine3 & 0.13501 & 0.13588 & 0.12861 & 0.12728 & 0.020151 & 0.030727 & 0.012376 & 0.0078105 \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.013867} & \textbf{0.016967} & \textbf{0.011242} & \textbf{0.008872} & \textbf{0.012997} & \textbf{0.01044} & \textbf{0.0034002} & \textbf{0.00069215} \\ \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \caption{N6V13-Validation}
% \label{tab:N6V13}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% N6V13                              & scene1(8)         & scene2(9)         & scene3(10)        & scene4(11)        & scene5(12)       & scene6(6)         & scene7(7)          & scene8(14)          \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline1  & 0.034218          & 0.033919          & 0.034647          & 0.034323          & 0.033304         & 0.03028           & 0.034507           & 0.028821            \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline2  & 0.14575           & 0.14111           & 0.14279           & 0.1409            & 0.035097         & 0.037736          & 0.034956           & 0.022531            \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.020817} & \textbf{0.023358} & \textbf{0.011638} & \textbf{0.011406} & \textbf{0.01137} & \textbf{0.012674} & \textbf{0.0027765} & \textbf{9.7622e-05} \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \caption{RealExp-Validation}
% \center
% \label{tab:RealExp}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
%  & Baseline1 & BaseLine3 & Our Method \\ \hline
% \cellcolor[HTML]{C0C0C0}RealExp & 0.0068 & 0.0082 & \textbf{0.0052} \\ \hline
% \end{tabular}
% \end{table*}














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \caption{}
% \label{tab:my-table}
% \center
% \resizebox{2.2\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
%  & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \hline
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0596 & -0.0406 & 0.0576 & 0.0361 & -0.0530 & -0.0489 & -0.0016 & 0.0230 & 0.0201 & -0.0337 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.0000 & -0.0000 & 0.0000 & -1.2201 & -0.0452 & 0.0271 & -0.4877 & -0.4553 & -0.0639 & 0.3249 & -0.0348 & -0.1575 & -0.1383 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.1006 & -0.0340 & 0.0370 & 0.0553 & -0.0517 & 0.0026 & -0.0065 & -0.0047 & -0.0144 & -0.0019 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0 & 0 & 0 & -2.7494 & 0.1256 & 0.3751 & -1.2767 & -0.4196 & 0.9424 & -1.6712 & 0.7878 & 0.1668 & 0.9364 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0157 & -0.0204 & 0.0265 & -0.0013 & -0.0465 & -0.0569 & -0.0156 & 0.0218 & 0.0162 & -0.0455 & -0.0332 & 0.0393 & 0.0222 & -0.0332 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & -0.0842 & -0.3518 & -0.0219 & -0.0202 & 0.0533 & -0.0017 & 0.0181 & 0.0277 & 0.0241 & -0.0009 & 0.0810 & 0.0146 & -0.2053 & -0.5344 & 0.0000 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & -0.0078 & 0.0122 & 0.0011 & -0.0001 & 0.0004 & -0.0010 & -0.0039 & -0.0005 & 0.0045 & 0.0043 & 0.0101 & 0.0072 & 0.0202 & -0.0511 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \multirow{-11}{*}{\cellcolor[HTML]{C0C0C0}Scene 1} & percentage & 0.4621 & 0.1934 & 0.9593 & 0.9409 & 0.9917 & 0.9815 & 0.7567 & 0.9761 & 0.7292 & 0.9050 & 0.7201 & 0.8199 & -0.0973 & -1.3641 & 0 & 0 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0596 & -0.0406 & 0.0576 & 0.0361 & -0.0530 & -0.0488 & -0.0016 & 0.0120 & 0.0103 & -0.0121 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.0000 & -0.0000 & 0.0000 & -1.2201 & -0.0452 & 0.0271 & -0.4877 & -0.4553 & -0.0614 & 0.3359 & 0.4624 & 0.4051 & 0.5910 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.1006 & -0.0340 & 0.0370 & 0.0553 & -0.0517 & -0.0444 & -0.0014 & -0.0029 & 0.0188 & -0.0018 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0 & 0 & 0 & -2.7494 & 0.1256 & 0.3751 & -1.2767 & -0.4196 & 0.0333 & 0.4237 & 0.8704 & -0.0862 & 0.9385 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0.0030 & -0.0009 & 0.0195 & 0.0094 & -0.0312 & -0.0530 & -0.0303 & 0.0271 & 0.0202 & -0.0600 & -0.0435 & 0.0476 & 0.0320 & -0.0332 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & 0.7948 & 0.9371 & 0.2491 & -6.5393 & 0.3660 & 0.0666 & -0.9079 & -0.2091 & -0.2136 & -0.3195 & -0.2029 & -0.1957 & -0.7393 & -0.5344 & 0.0000 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & -0.0135 & 0.0121 & 0.0230 & -0.0001 & 0.0004 & -0.0505 & -0.0039 & 0.0200 & 0.0045 & -0.0393 & -0.0381 & 0.0072 & 0.0142 & -0.0511 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 2\\ (9)\end{tabular}} & percentage & 0.0686 & 0.1977 & 0.1152 & 0.9464 & 0.9913 & 0.1117 & 0.7569 & 0.1074 & 0.7292 & 0.1361 & -0.0535 & 0.8195 & 0.2284 & -1.3641 & 0 & 0 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0596 & -0.0431 & 0.0603 & 0.0160 & -0.0334 & -0.0528 & -0.0069 & 0.0141 & 0.0159 & -0.0225 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.0000 & -0.0000 & 0.0000 & -1.2201 & -0.1083 & -0.0174 & 0.3405 & 0.0846 & -0.1485 & -1.8363 & 0.3677 & 0.0816 & 0.2406 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.1006 & -0.0078 & 0.0251 & -0.0008 & 0.0004 & 0.0009 & -0.0034 & 0.0155 & -0.0024 & 0.0030 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0 & 0 & 0 & -2.7494 & 0.7980 & 0.5758 & 0.9688 & 0.9895 & 0.9801 & -0.3877 & 0.3043 & 0.8612 & 0.8990 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0127 & -0.0255 & 0.0181 & -0.0034 & -0.0496 & -0.0563 & -0.0155 & 0.0241 & 0.0129 & -0.0607 & -0.0476 & 0.0604 & 0.0271 & -0.0433 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & 0.1182 & -0.6921 & 0.3030 & -1.7154 & -0.0085 & 0.0086 & 0.0273 & -0.0737 & 0.2238 & -0.3354 & -0.3174 & -0.5152 & -0.4713 & -1.0034 & 0.0000 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0.0017 & 0.0033 & 0.0006 & 0.0003 & -0.0004 & -0.0578 & -0.0001 & -0.0001 & 0.0005 & 0.0000 & -0.0000 & 0.0431 & -0.0000 & -0.0475 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 3\\ (10)\end{tabular}} & percentage & 0.8852 & 0.7822 & 0.9781 & 0.7585 & 0.9925 & -0.0178 & 0.9915 & 0.9950 & 0.9699 & 0.9996 & 0.9989 & -0.0816 & 0.9976 & -1.1978 & 0 & 0 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0596 & -0.0406 & 0.0563 & 0.0376 & -0.0520 & -0.0477 & -0.0002 & 0.0275 & 0.0242 & -0.0335 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.0000 & -0.0000 & 0.0000 & -1.2201 & -0.0452 & 0.0498 & -0.5483 & -0.4264 & -0.0384 & 0.9218 & -0.2351 & -0.3963 & -0.1328 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0283 & -0.0480 & -0.0346 & -0.0029 & 0.0027 & -0.0017 & 0.0033 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0 & 0 & 0 & 0 & 0 & 0 & -0.1642 & -0.3174 & 0.2473 & -0.2098 & 0.8785 & 0.9013 & 0.8902 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0172 & -0.0186 & 0.0292 & 0.0015 & -0.0472 & -0.0547 & -0.0166 & 0.0215 & 0.0180 & -0.0436 & -0.0323 & 0.0339 & 0.0062 & -0.0461 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & -0.1874 & -0.2343 & -0.1270 & -0.2300 & 0.0387 & 0.0362 & -0.0413 & 0.0407 & -0.0793 & 0.0407 & 0.1068 & 0.1486 & 0.6629 & -1.1330 & 0.0000 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0.0015 & 0.0033 & 0.0007 & -0.0002 & -0.0003 & -0.0003 & -0.0001 & -0.0007 & 0.0005 & 0.0001 & -0.0001 & 0.0005 & 0.0060 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 4\\ (11)\end{tabular}} & percentage & 0.8978 & 0.7778 & 0.9726 & 0.8257 & 0.9938 & 0.9947 & 0.9965 & 0.9704 & 0.9680 & 0.9979 & 0.9962 & 0.9882 & 0.6754 & 0 & 0 & 0 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 0.0242 & -0.0335 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0517 & -0.0411 & 0.0563 & 0.0388 & -0.0564 & -0.0481 & -0.0025 & 0.0197 & 0.0229 & -0.0392 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.0000 & -0.0000 & 0.0000 & -0.9248 & -0.0584 & 0.0493 & -0.5974 & -0.5477 & -0.0464 & -0.0365 & 0.1148 & -0.3199 & -0.3244 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0822 & -0.0249 & 0.0195 & -0.0236 & 0.0063 & 0.0090 & -0.0135 & -0.0055 & -0.0128 & -0.0052 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0 & 0 & 0 & -2.0617 & 0.3584 & 0.6704 & 0.0259 & 0.8270 & 0.8044 & -4.5801 & 0.7537 & 0.2643 & 0.8244 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0181 & -0.0260 & 0.0242 & -0.0005 & -0.0451 & -0.0526 & -0.0151 & 0.0262 & 0.0125 & -0.0462 & -0.0340 & 0.0416 & 0.0128 & -0.0318 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & -0.2515 & -0.7232 & 0.0686 & 0.6020 & 0.0822 & 0.0741 & 0.0518 & -0.1665 & 0.2474 & -0.0159 & 0.0577 & -0.0443 & 0.3057 & -0.4699 & 0.0000 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & -0.0094 & 0.0087 & 0.0006 & 0.0001 & 0.0002 & 0.0022 & -0.0038 & 0.0001 & 0.0040 & 0.0042 & 0.0102 & 0.0436 & -0.0202 & -0.0044 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 5\\ (12)\end{tabular}} & percentage & 0.3470 & 0.4238 & 0.9776 & 0.9165 & 0.9952 & 0.9613 & 0.7596 & 0.9945 & 0.7602 & 0.9072 & 0.7165 & -0.0955 & -0.0947 & 0.7942 & 0 & 0 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0287 & -0.0521 & -0.0570 & -0.0040 & 0.0034 & -0.0057 & -0.0260 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.0000 & -0.0000 & 0.0000 & -0.0000 & 0 & -0.0000 & -0.1815 & -0.4313 & -0.2419 & -0.6623 & 0.8473 & 0.6698 & 0.1209 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & -0.0177 & 0.0002 & -0.0001 & 0.0001 & -0.0000 & -0.0001 & -0.0002 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0 & 0 & 0 & 0 & 0 & 0 & 0.2714 & 0.9957 & 0.9984 & 0.9773 & 0.9992 & 0.9958 & 0.9938 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0078 & -0.0121 & 0.0162 & -0.0046 & -0.0302 & -0.0391 & -0.0105 & 0.0209 & 0.0049 & -0.0302 & -0.0251 & 0.0415 & 0.0175 & -0.0483 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & 0.4595 & 0.1946 & 0.3746 & -2.6458 & 0.3855 & 0.3123 & 0.3384 & 0.0693 & 0.7074 & 0.3352 & 0.3047 & -0.0412 & 0.0473 & -1.2325 & 0.0000 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0.0005 & -0.0000 & 0.0052 & -0.0013 & -0.0000 & 0.0001 & 0.0000 & 0.0002 & -0.0000 & -0.0003 & 0.0000 & -0.0000 & -0.0007 & -0.0690 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 6\\ (6)\end{tabular}} & percentage & 0.9646 & 1.0000 & 0.7986 & -0.0668 & 0.9994 & 0.9980 & 0.9999 & 0.9899 & 0.9999 & 0.9937 & 1.0000 & 1.0000 & 0.9633 & -2.1906 & 0 & 0 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0000 & 0.0001 & 0.0006 & 0.0016 & -0.0367 & 0.0568 & 0.0322 & -0.0443 & -0.0308 & 0.0006 & 0.0265 & 0.0217 & -0.0278 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.9995 & 0.9910 & 0.9915 & 0.9394 & 0.0546 & 0.0414 & -0.3251 & -0.2164 & 0.3303 & 0.7327 & -0.1897 & -0.2511 & 0.0610 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & -0.0000 & -0.0000 & 0.0000 & -0.0000 & -0.0000 & -0.0000 & -0.0052 & 0.0041 & -0.0022 & -0.0016 & 0.0001 & -0.0000 & 0.0017 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 1.0000 & 0.9997 & 1.0000 & 0.9986 & 0.9999 & 1.0000 & 0.7874 & 0.8884 & 0.9515 & 0.3296 & 0.9934 & 0.9984 & 0.9423 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0063 & -0.0377 & 0.0166 & -0.0125 & -0.0458 & -0.0593 & -0.0302 & 0.0257 & 0.0259 & -0.0379 & -0.0283 & 0.0342 & 0.0122 & -0.0307 & 0.0202 & -0.0081 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & 0.5655 & -1.4996 & 0.3586 & -8.9781 & 0.0686 & -0.0446 & -0.8992 & -0.1445 & -0.5561 & 0.1658 & 0.2179 & 0.1428 & 0.3389 & -0.4222 & 0.6702 & 0.7643 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0.0003 & 0.0002 & 0.0001 & -0.0002 & -0.0000 & -0.0001 & -0.0003 & -0.0003 & 0.0003 & 0.0002 & -0.0361 & -0.0005 & 0.0012 & -0.0018 & 0.0007 & 0.0000 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 7\\ (7)\end{tabular}} & percentage & 0.9778 & 0.9850 & 0.9974 & 0.8430 & 0.9990 & 0.9977 & 0.9804 & 0.9864 & 0.9846 & 0.9947 & -0.0000 & 0.9880 & 0.9367 & 0.9174 & 0.9891 & 0.9997 \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & 0 & 0 & 0 & 0.0284 & 0.0106 & -0.0710 & 0.0268 & -0.0388 & 0.0592 & 0.0243 & -0.0364 & -0.0459 & -0.0024 & 0.0222 & 0.0173 & -0.0296 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & 0 & 0 & 0 & 0.0000 & 0.0001 & 0.0006 & 0.0016 & -0.0367 & 0.0568 & 0.0299 & -0.0425 & -0.0412 & 0.0006 & 0.0200 & 0.0260 & -0.0194 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.9286 & 0.2615 & -0.2238 & -0.4113 & -0.0445 & 0.0529 & -0.8577 & -0.6922 & -0.2556 & 0.9480 & 0.2625 & 0.0379 & 0.4167 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0 & 0 & 0 & -0.0000 & -0.000003 & 0.000001 & -0.0000364 & -0.0000032 & -0.0009000 & 0.0000002 & -0.0000 & -0.0000012 & 0.0000447 & -0.0000001 & -0.0000002 & 0.0000 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & NaN & NaN & NaN & 0.8128 & 0.9998 & 1.0000 & 0.9994 & 1.0000 & 0.9998 & 0.9956 & 0.9919 & 0.9987 & 1.0000 & 1.0000 & 0.9998 & 1.0000 \\ \cline{2-18} 
% \rowcolor[HTML]{C0C0C0} 
% \cellcolor[HTML]{C0C0C0} & No. ring & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Origin & -0.0145 & -0.0151 & 0.0259 & -0.0013 & -0.0491 & -0.0568 & -0.0159 & 0.0224 & 0.0166 & -0.0454 & -0.0361 & 0.0398 & 0.0184 & -0.0216 & 0.0612 & -0.0344 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & BaseLine & -0.0058 & -0.0244 & 0.0188 & -0.0044 & -0.0380 & -0.0456 & -0.0149 & 0.0211 & 0.0138 & -0.0409 & -0.0358 & 0.0314 & 0.0168 & -0.0062 & 0.0304 & -0.0081 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & percentage & 0.5693 & -0.5067 & 0.2980 & -2.5661 & 0.2070 & 0.2531 & 0.0279 & 0.0983 & 0.1802 & 0.0613 & 0.0583 & 0.0169 & -0.4188 & 0.5644 & -0.6370 & 0.0493 \\ \cline{2-18} 
% \cellcolor[HTML]{C0C0C0} & Our Method & 0.0000 & -0.000007 & 0.000002 & 0.0000005 & 0.0000057 & 0.0000002 & 0.0000091 & 0.0000004 & 0.0000001 & -0.0000005 & 0.0000269 & -0.0000002 & -0.0000 & -0.0003148 & 0.0000028 & 0.0000095 \\ \cline{2-18} 
% \multirow{-12}{*}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Scene 8\\ (14)\end{tabular}} & percentage & 0.9996 & 1.0000 & 0.9995 & 0.9984 & 0.9986 & 1.0000 & 0.9999 & 0.9999 & 1.0000 & 0.9998 & 0.9998 & 1.0000 & 0.9996 & 1.0000 & -0.0084 & 0.6589 \\ \hline
% \end{tabular}
% }
% \end{table*}


% \begin{table*}[]
% \caption{}
% \label{tab:my-table}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
%  & scene1(8) & scene2(9) & scene3(10) & scene4(11) & scene5(12) & scene6(6) & scene7(7) & scene8(14) \\ \hline
% \cellcolor[HTML]{C0C0C0}Baseline & 0.0304 & 0.0296 & 0.0308 & 0.0304 & 0.0303 & 0.0255 & 0.0222 & 0.0285 \\ \hline
% \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.02} & \textbf{0.026} & \textbf{0.0163} & \textbf{0.0152} & \textbf{0.0163} & \textbf{0.0133} & \textbf{0.0018} & \textbf{0.0025} \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% NoiseModel3Validate13 & scene1(8) & scene2(9) & scene3(10) & scene4(11) & scene5(12) & scene6(6) & scene7(7) & scene8(14) \\ \hline
% Baseline1 & 0.027746 & 0.028385 & 0.02513 & 0.025884 & 0.026573 & 0.027339 & 0.030523 & 0.026707 \\ \hline
% BaseLine2 & 0.043125 & 0.068242 & 0.049517 & 0.046253 & 0.046174 & 0.029587 & 0.060347 & 0.03716 \\ \hline
% Our Method & 0.034402 & 0.029771 & 0.029218 & 0.029035 & 0.031913 & 0.035527 & 0.04056 & 0.036853 \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% NoiseModel6Validate13 & scene1(8) & scene2(9) & scene3(10) & scene4(11) & scene5(12) & scene6(6) & scene7(7) & scene8(14) \\ \hline
% Baseline1 & 0.019121 & 0.019153 & 0.016667 & 0.018322 & 0.017758 & 0.020595 & 0.023881 & 0.020254 \\ \hline
% BaseLine2 & 0.060039 & 0.13258 & 0.030624 & 0.032082 & 0.033106 & 0.019022 & 0.023475 & 0.021776 \\ \hline
% Our Method & 0.023161 & 0.020851 & 0.016321 & 0.024645 & 0.022655 & 0.019756 & 0.024101 & 0.026319 \\ \hline
% \end{tabular}
% \end{table*}



% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
%  & scene1(8) & scene2(9) & scene3(10) & scene4(11) & scene5(12) & scene6(6) & scene7(7) & scene8(14) \\ \hline
% Baseline1 & 0.028716 & 0.029088 & 0.027749 & 0.027051 & 0.029204 & 0.026915 & 0.025437 & 0.029001 \\ \hline
% BaseLine2 & 0.063847 & 0.078926 & 0.042745 & 0.038572 & 0.046011 & 0.030332 & 0.036107 & 0.028396 \\ \hline
% Our Method & 0.030856 & 0.039806 & 0.037244 & 0.033635 & 0.04556 & 0.036004 & 0.036501 & 0.029569 \\ \hline
% \end{tabular}
% \end{table*} 

==> Experiments.tex <==
\section{Experimental and Simulation Results}
\label{sec:SimulationResults}
This section first presents a simulation study of the intrinsic calibration problem
that will show the importance of properly constructed scenes for eliminating over
parameterization in two of the three calibration models. Results here will be used to
inform the experimental work. All experiments are conducted from a \velodyne and an
\textit{Intel RealSense Depth Camera D435}, mounted on an in-house designed torso for
a Cassie-series bipedal robot~\cite{CassieAutonomy2019ExtendedEdition}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulated \lidar Environment}
\label{sec:Simulator}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Due to lack of ground truth, we built a \lidar simulator from scratch to compare our
calibration method against two baselines and to illustrate the role of target
positioning in the construction of a calibration environment. As an example of the
latter, Fig.~\ref{fig:PropositionIllustration} illustrates a scene where a unique
solution does not exist for two of the three calibration models, namely,
\eqref{eq:OptSolution} and \eqref{eq:ComplexCalibration}. Our simulator can model
\lidar sensors of different working principles (spinning vs solid-state). With our
simulator, it is easy to control sources of uncertainty, including both mechanical
model uncertainty and measurement noise. Targets are assumed to be planar and
polygonal.

To simulate 3D points on a planar target, we generate rays from the \lidar sensor,
and define a ``target'' point as the point at which the ray intersects the target.
The simulator has an option to account for shadowing or not. After locating the exact
\lidar returns on the target, based on the \lidar type, we then add two types of
uncertainty to the returns and report them as measured data. 

\begin{remark} 
    The simulator first finds all intersection points with the (infinite) plane
    defined by the target.  To determine if a point on the plane is within the
    boundary of the target polygon is a \add{well-known} problem in computer
    graphics, called the Point-In-Polygon (PIP) problem. The Winding Number algorithm
    \cite{alciatore1995winding} is implemented in this simulator. If the winding
    number of a point is not zero, the point lies inside the boundary; otherwise it
    is outside. 
\end{remark}

\subsection{Calibration Scenes}
\label{sec:AdequateEnvironment}
 To illustrate Theorem~\ref{thm:uniqueness} and the role of target selection and
 placement in the case of a spinning \lidarN, we define five different scenes, where
 five will be used for ``training'' and one will be used for ``validation''. Because
 the calibration is being conducted for a spinning \lidarN, the points are parsed
 ``per ring'' as discussed in Sec.~\ref{sec:IntrinsicCalibration}. The target sizes
 vary with distance to ensure a minimum of ten points per ring on each target.


\begin{table*}[t]
    \caption{\bh{Check again}Induce 3-parameter perturbation model $(\N[1])$,  6-parameter perturbation
model $(\N[2])$, and $\Sim(3)$ noise model $(\N[3])$ for a spinning \lidar in the
simulator. The error is the P2P cost in meter and validated in a complex scene.} 
\label{tab:N3}
\center
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\cellcolor[HTML]{C0C0C0}Noise Model &\cellcolor[HTML]{C0C0C0} Methods & \cellcolor[HTML]{C0C0C0}scene 1 & \cellcolor[HTML]{C0C0C0}scene 2 & \cellcolor[HTML]{C0C0C0}scene 3 & \cellcolor[HTML]{C0C0C0}scene 4 & \cellcolor[HTML]{C0C0C0}scene 5 & \cellcolor[HTML]{C0C0C0}scene 6 \\ \hline
\cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline1 & 0.036998 & 0.037076 & 0.034804 & 0.032165 & 0.017921 & 0.028471 \\ \cline{2-8} 
\cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline2 & 0.16108 & 0.15412 & 0.15745 & 0.035424 & 0.023221 & 0.023275 \\ \cline{2-8} 
\multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}N1} & \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.020421} & \textbf{0.028072} & \textbf{0.013583} & \textbf{0.010428} & \textbf{0.0016329} & \textbf{0.0010792} \\ \hline
\cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline1 & 0.024689 & 0.025205 & 0.027227 & 0.021967 & 0.010316 & 0.012955 \\ \cline{2-8} 
\cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline2 & 0.14897 & 0.14993 & 0.14192 & 0.033905 & 0.012305 & 0.0086185 \\ \cline{2-8} 
\multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}N2} & \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.015302} & \textbf{0.018722} & \textbf{0.012405} & \textbf{0.01152} & \textbf{0.003471} & \textbf{0.00076376} \\ \hline
\cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline1 & 0.037758 & 0.037428 & 0.038231 & 0.033412 & 0.023682 & 0.031802 \\ \cline{2-8} 
\cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0}Baseline2 & 0.16082 & 0.15571 & 0.15756 & 0.04164 & 0.022272 & 0.024862 \\ \cline{2-8} 
\multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}N3} & \cellcolor[HTML]{C0C0C0}Our Method & \textbf{0.02297} & \textbf{0.025774} & \textbf{0.012842} & \textbf{0.013986} & \textbf{0.0053697} & \textbf{0.00010772} \\ \hline
\end{tabular}
\end{table*}

\begin{itemize} 
    \item \bh{check all the scenes again.}Scene 1: Two targets are placed along the same side of the $x$-axis, parallel
    to each other and to the $z$-axis .
\item Scene 2: Two targets are placed at different distances and opposite sides along
    the $x$-axis of the \lidarN, parallel to one another and to the $z$-axis.
\item Scene 3: Four targets are placed at right angles. This models the use the
    common use of vertical walls for calibration. 
\item Scene 4: It is a complex scene for validation. Eight targets are placed at
    various distance and orientations. Four of them are close the LiDAR and the other
    four are far from LiDAR.
\item Scene 5: We place 12 targets at different distances with various angles. 
\item Scene 6: We place 24 targets at different distances with various angles. 
\end{itemize}


% \begin{itemize} 
% \item Scene 1: two targets are placed at equal distance and opposite sides along the
%     $x$-axis of the \lidarN, parallel to one another and to the $z$-axis ($\n[1],
%     \n[2]$ are not \lind). 
%     \item Scene 2: two targets are placed at right angles and
%     one slightly tilted up ($\n[1], \n[2], \n[3]$ are mathematically \lind, but have a poor condition number\footnote{In the sense of their SVD.}. In practice, this will lead to poor calibration results). 
% \item Scene 3: four targets are placed at right angles. This models the use the common use of vertical walls for calibration. This calibration scene will break the uniqueness constraints and thus lead to poor calibration results.
% \item Scene 4 : two targets are placed at right angles and one tilted up at $45^\circ$ angle ($\n[1], \n[2], \n[3]$ are \lind and well conditioned). We deliberately avoid passing a beam through $q_0$ in \eqref{eq:PoleOfCalibration}.
% \item Scene 5 : a complex scene for validation. We place eight targets at different
% distances with various angles. 
% \end{itemize}

\begin{remark}
    The placement of only a few targets in a scene is done to demonstrate the ``minimum''
requirements to calibrate a spinning \lidarN. One can place as many targets as desired in
the simulator. 
\end{remark}

\begin{figure}[b]%
\centering
\subfloat{%
\label{fig:NormalsVSP2P}%
\includegraphics[width=0.95\columnwidth, trim={0cm 7cm 0cm 0cm},clip]{placeholder.png}}\\
\subfloat{%
    \label{fig:OrientationVSP2P}%
\includegraphics[width=0.95\columnwidth, trim={0cm 7cm 0cm 0cm},clip]{placeholder.png}}
\caption[]{\bhp{}}
\label{fig:P2PResults}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\lidar Intrinsic Calibration of a Spinning \lidar}
\label{sec:SimSpingHead}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For each scene, we generate deterministic measurements by applying the following
perturbations to the data on a per-ring basis (i.e, values vary by ring number): (i)
simple model $(\drho, \dtheta, \dphi)$, (ii) complex model $(\drho, \dtheta, \dphi,
s, h, v)$, and (iii) $\Sim(3)$ model $(\R, \t, s)$, denoted as $\N[1], \N[2], \N[3]$,
respectively. The exact values used are in a \texttt{.mat} file uploaded to GitHub
\cite{githubFileIntrinsic}. For each target, its true normal vector $\n$ and point
$\p[0]$ on the target are assumed known so that the P2P cost functions can be
evaluated. For each of the three cost functions \eqref{eq:OptSolution},
\eqref{eq:SimpleCalibration}, \eqref{eq:ComplexCalibration}, the \texttt{fmincon}
function in MATLAB is used to determine calibration parameters achieving a local
minimum for each Scene. The initializations for \texttt{fmincon} are selected to
correspond to zero perturbation error, that is the parameters are zero, one or the
identify matrix as the case requires. The optimized calibration parameters are then
applied to the data of Scene 5 and the P2P cost of \eqref{eq:OptSolution} is
evaluated and reported as validation data in Table~\ref{tab:N3}.

The simulated results confirm that a single target results in degeneracy when
calibrating with the $\BL_2$ and $\Sim(3)$ models, and while $\BL_1$ works fine with
a single target, it drops in performance as the complexity of the calibration errors
is increased. The well-posedness of the $\BL_2$ and $\Sim(3)$ calibration models was
confirmed when the conditions of Theorem.~\ref{thm:uniqueness} are respected.

\addd{To further analyze the proposed method and verify Theorem~\ref{thm:uniqueness},
    we consider the following two scenarios: \textbf{1)} We generate \bh{10 thousand}
    training scenes in which we randomly place 4 targets at different
    distances with various angles. \textbf{2)} We generate 10 thousand training
    scenes in which we randomly rotate the tetrahedron, as shown in
    Fig.~\ref{fig:oriented-tetrahedron}. We compute the condition number of normal
    vectors (Assumption~\ref{asm:assumtionN}), and the condition number of bases
    (Assumption~\ref{asm:assumtionB}) for both scenarios. The optimized calibration
    parameters are then applied to the data of Scene 5 and the P2P cost of
\eqref{eq:OptSolution} is evaluated. The results are reported in
Fig.~\ref{fig:P2PResults}. Again, we can
see, as expected, when the condition number of normal vectors
worsens, the validation P2P cost increases. However, when the condition number of bases increases, the
P2P cost does not increase as we expected. Therefore, in practice, 
a set of well-conditioned target's normal vectors is sufficient to calibrate a
\slidarN.}





% \textbf{\bh{TBD} These are the OLD Key Findings:}
% \begin{enumerate}
%     \item The proposed method performs well. 
%     \item Table \bh{} shows that the $\BL_1$ has constant performance. This is
% because it requires a simple target arrangement suffices to uniquely determine its
% calibration parameters. On the other hand, \BL2 and $\Sim(3)$ require more complex
% geometries to uniquely determine their parameters and thereby avoid overfitting. In
% Table \bh{??}, even though $\BL_1$ does not have enough parameters to represent the
% perturbations in the data, its validation error does decrease as the scene geometry
% becomes more rich. As in Table~\bh{one}, the early scenes do not provide enough
% information to uniquely determine the parameters in $\BL2$ and $\Sim(3)$, as compared
% to the later scenes. These trends are continued in Table~\bh{??}. 
% \end{enumerate}

\subsection{\lidar Intrinsic Calibration of a Solid State \lidar}
\label{sec:ExpSSLiDAR}
An OPA \sslidar is fabricated on a planar wafer with a large number of emitters, see
Sec.~\ref{sec:intro}. We induce geometric uncertainty into the system by assuming the
plane of the wafer is slightly warped. In the simulator, the OPA \sslidar has
$20\times20$ emitters with 160, 40 horizontal and vertical field of view,
respectively. We place four targets of the same size.
\addd{Theorem~\ref{thm:uniqueness} requires a ring plane, as mentioned in
    Sec.~\ref{sec:TargetPlacementGuideline}. We therefore parse the \lidar returns to
an $20\times4$ uniform grid over the planar targets, so each of the grids can form its
own ring plane. This results in a total of 80 calibration models.} For each grid, the
cost function \eqref{eq:OptSolution} is optimized using the \texttt{fmincon} function
in MATLAB to determine calibration parameters achieving a local minimum. The
calibrated sensor is then validated on the other four scenes that have different
angles and distances. The mean P2P cost of \eqref{eq:OptSolution} improves 37\%, and
the result is shown in Fig.~\bh{fig:sslidar}.
% \add{
% \begin{remark}
% Due to the warped wafer, the closer to the edge of the wafer, the larger the
%     distortion is. We therefore estimate the target's normal by weighted least
%     squares where the weight is the distance of each point to the mean of all the
%     points on the target. 
% \end{remark}
% }

\begin{figure}[t]%
\centering
\includegraphics[width=0.75\columnwidth, trim={0.5cm 1.0cm 0cm 1.5cm},clip]{validation-objs.jpg}
\caption{\bhi{}}
\label{fig:sslidar}%
\end{figure}

\begin{table}[t]
\caption{\bh{check all the scenes again.} Geometric uncertainty of a \sslidar by assuming the plane of the wafer is slightly warped.}
\label{tab:sslidar}
\center
\resizebox{\columnwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{C0C0C0}}c |c|c|c|}
\hline
Solid-State LiDAR & \cellcolor[HTML]{C0C0C0}Before Calibration & \cellcolor[HTML]{C0C0C0}After Calibration & \cellcolor[HTML]{C0C0C0}Improvement \\ \hline
Training results & 0.3315 & 0.0029 & 99.12 \% \\ \hline
Validation Scene1 & 0.2659 & 0.0197 & 92.59 \% \\ \hline
Validation Scene2 & 0.3193 & 0.0323 & 89.89 \% \\ \hline
Validation Scene3 & 0.2958 & 0.0202 & 93.16 \% \\ \hline
\end{tabular}
}
\end{table}


% \begin{table}[t]
% \caption{\bh{CHANGE. This is an old table using all 39 targets.} Experimental results of the automatic intrinsic calibration with targets arranged to avoid the degeneracies indicated in Prop.~\ref{thm:HopefullyTrue}.}
% \center
% \label{tab:RealExp}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0}
%  & Baseline1 & Baseline2 & Our Method \\ \hline
% \cellcolor[HTML]{C0C0C0}Validation Results & 0.0068 & 0.0082 & \textbf{0.0052} \\ \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[]
\caption{Experiments data collected using different numbers of targets in the calibration scene.}
\label{tab:RealExp}
\center
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0}
{\color[HTML]{000000} No.Tags} & 4 & 8 & 12 & 24 \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Baseline1} & \textbf{0.0064} & \textbf{0.0066} & 0.0066 & 0.0068 \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Baseline2} & 0.0146 & 0.0103 & 0.0083 & 0.0082 \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Our Method} & {\color[HTML]{000000} 0.0201} & {\color[HTML]{000000} 0.0084} & {\color[HTML]{000000} \textbf{0.0062}} & {\color[HTML]{000000} \textbf{0.0052}} \\ \hline
\end{tabular}
\end{table}

% \begin{figure}[t]%
% \centering
% \subfloat{%
% \label{fig:sslidarv1}%
% \includegraphics[width=0.75\columnwidth, trim={0.5cm 1.0cm 0cm 1.5cm},clip]{validation-objs.jpg}} \\
% % \hspace{2pt}%
% \subfloat{%
% \label{fig:sslidarv2}%
% \includegraphics[width=0.75\columnwidth, trim={1.5cm 1.0cm 0cm 4cm},clip]{validation-obj2-1.jpg}}~
% \caption[]{Left figure shows the placement of the validation scene. On the right shows one of the three validation results for OPA \sslidarN. The red dots indicates the calibrated \sslidar returns and the ``warped'' curvature is the noisy measurement.}% 
% \label{fig:sslidarv}%
% \end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiments of Intrinsic Calibration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:EXPIntrinsicCalibration}
Informed by the simulation study, a set of \lidar data was collected using the
\lidart package\cite{githubFileLiDARTag,huang2019lidartag} with targets arranged to
avoid the degeneracies indicated in Theorem~\ref{thm:uniqueness}. The targets' normal
vectors are estimated using the L1-inspired method in \cite{huang2020improvements}.
All together, 39 targets were collected as potential training data. On a separate
day, an additional 12 targets were collected for validation. Table~\ref{tab:RealExp}
reports validation data for the three calibration methods on various subsets of the
targets based on number of targets: four, seven, 10 of them.

It is seen that the trends observed in the simulation data for a spinning \lidar
continue to hold in experiments. We conclude that the proposed idea of reformulating
the calibration problem in terms of shape-preserving transformations on the observed
point cloud has been supported (i.e., not invalidated). With the open-source release
of our code and data, it will be straightforward for other groups to confirm or deny
this finding.



==> Introduction_.tex <==
\section{Introduction and Contributions}
\label{sec:intro}
Camera and Light Detection And Ranging (\lidarN) are common sensors for current
robotics and autonomous systems. For real-world operations, the performance of such
systems highly depends on the quality of intrinsic and extrinsic calibration
parameters. 
Intrinsic calibration of a sensor is the process of ensuring that obtained
measurements are meaningful and valid. Intrinsic calibration of a camera is
relatively mature and open-sourced packages are available~\cite{maye2013self,
itseez2015opencv, quigley2009ros}. In this work, we are concerned with the problem of
multi-beam \lidar intrinsic calibration. We focus on narrow-pulsed time of flight
(ToF) method: spinning \lidars and \sslidarsN, as shown in Fig.~\ref{fig:FirstImage}.
\addd{Figure~\ref{fig:SystematicError} shows a factory-calibrated high-end \lidar
(\velodyneN) measuring a planer target.} \add{The measurements are not consistent (mis-calibrated
    rings) and result in a point cloud with \bh{7 cm} thickness.
}

\jwg{Bruce will create tension! See writing video.}

\subsection{Spinning \lidar}
A spinning \lidar as used in this paper consists of $K$ laser emitter-receiver pairs
mounted at various positions and elevation angles on the rotating head, as shown in
Fig.~\ref{fig:FirstImage}. The lasers are pulsed at a fixed frequency. Each
revolution of the rotating head sweeps out a cone in space, called a \lidar scan,
composed of discrete return points traced out by each pulsed emitter-receiver. The
points associated with a single laser beam are also called a ring. 

The measurements are typically viewed as being made in a spherical coordinate system.
The range measurement is made by estimating ToF through a clocking system on a
circuit board, the azimuth is estimated from the position of the rotating head, and
the elevation angle of a beam is determined by its mounting angle on the rotating
head. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{FirstFigure.png}
\caption{This figure motivates the main contribution of the
    paper, a means of calibrating a \lidar without modeling the physical mechanism
    itself. Top left: shows a simple physics-based calibration model for a spinning
    \lidarN. Top right: shows a similar model with more parameters, also for a spinning
    \lidarN. In the literature, the number of parameters can vary from three to 10.
    Bottom left and bottom right show, respectively, an optical phased array \sslidar and a
    MEMS-based \sslidarN. There are many design options and many manufacturing steps
    to fabricate these \lidars. Is it necessary, or even possible, to parameterize
    all of them? This paper moves the attention to the geometry of the \lidarN's
    point cloud  and proposes that calibration can be achieved via shape-preserving
    transformations. 
    In experiments, the proposed method outperforms the methods showed in top figures
for spinning \lidarsN, and via simulation, we support that it may be used to
calibrate \sslidars as well.} 
\label{fig:FirstImage}
\squeezeup
\squeezeup
\end{figure}

\begin{figure}[t]%
\centering
\subfloat{%
\includegraphics[height=0.65\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{BeforeCalibration.png}} 
\hfill
\subfloat{%
\includegraphics[height=0.65\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{AfterCalibration.png}}~
\caption[]{On the left shows a factory-calibrated \velodyne measuring on a planer
    target. The measurements are not consistent and lead to a thickness of \bh{7 cm} point
cloud with \bh{4 cm} P2P distance. On the right shows the calibration results for the
proposed method. The thickness and P2P distance after calibration are \bh{3 cm} and
\bh{0.002 cm}.}%
\label{fig:SystematicError}%
\end{figure}


Existing error models for \lidars are phenomenological in nature, that is, they are
tied to physical explanations of a sensor's design and/or
operation~\cite{mirzaei20123d,pandey2010extrinsic,glennie2010static,
nouira2016point,chan2013temporal,atanacio2011lidar,
muhammad2010calibration,bergelt2017improving}. Broadly speaking, two sources of
uncertainty are typically considered in spinning \lidar models: (1) errors in the
clocking systems, (one for ToF and one for pulsing the lasers) and (2) mechanical
errors associated with positioning of the beams on the spinning \lidarN. Some authors
overlook that the measurements are actually made in a local coordinate frame for each
emitter-receiver pair, and are then transformed to a single ``global'' frame for the
\lidar unit, resulting in models with three to six parameters
\cite{pandey2010extrinsic, muhammad2010calibration, glennie2010static}, while others
take this into account and use as many as ten parameters~\cite{bergelt2017improving}.
Moreover, none of these models provides a guideline for target placement so that
the calibration model is well-constrained (i.e., a unique solution exists), see
Sec.~\ref{sec:TargetPlacementGuideline}.


\subsection{Solid-State \lidar}
\label{sec:SolidStateLiDAR}
In comparison  to spinning \lidarsN, \sslidars are smaller, quieter, lower-cost, and
produce less vibration. Several types of \sslidar are coming to the market, including
those based on (1) Optical Phased Array (OPA) \cite{frederiksen2020lidar,
poulton2019long, poulton2018high}, and (2) Micro-Electro-Mechanical System (MEMS)
mirrors\footnote{Some authors argue MEMS-based \sslidars are not truly solid-state
devices due to the movable mirrors; the mirrors, however, are tiny compared to a
spinning \lidarN.}\cite{yoo2018mems, pelz2020matrix, druml20181d, lee2015optical}. 

OPA-based \sslidars function similarly to a phased array in antenna theory. A single
OPA contains a significant number of emitters patterned on the chip. By varying the
phase shift (i.e., time delay) of each emitter, the direction of the resulting
wave-front or the spread angle can be adjusted. In particular, the sensor is able to
zoom in or out of an object on command. On the other hand, MEMS-based \sslidars use
only one or a few emitters, with the beams guided by a mirror system regulated by a
sophisticated controller. The controller seeks to steer the beam (or beams) in a
scanning pattern, such as a zig-zag \cite{yoo2018mems}. 

To perfectly align OPA emitters or MEMS mirrors is challenging. It is also hard to
maintain high accuracy under different temperatures and weather conditions. Thus, how
to properly calibrate a \sslidar is a critical problem.

The variety of \sslidars raises the question: is it necessary, or even possible, to
design/create parameterized models for every type of \sslidarN? This paper seeks to
present a unifying view of \lidar calibration by abstracting away from the physics of
a \lidar type (spinning vs solid state, for example), and focusing instead on the
spatial geometry of the point cloud generated by the sensor. This leads to a unifying
view of calibration. 


\subsection{Our Contributions}
\label{sec:Contributions}
\begin{enumerate}
   
     \item We propose a model for intrinsic \lidar calibration that is independent of the underlying technology. The new error model is based on
         shape-preserving transformations\footnote{Called \textit{similarity
         transformations} in projective geometry.}, that is a rigid body
         transformation plus a scale factor. Currently, intrinsic calibration models
         exist only for spinning LiDARs. The calibration models are tied to
         postulated physical mechanisms for how the \lidar functions, resulting in
         anywhere from three to ten parameters to be estimated from data. Instead, we
         \textit{abstract away from the physics of a \lidar type} (spinning head vs
         solid state, for example) and focus on the spatial geometry of the point
         cloud generated by the sensor. \textit{This leads to a unifying view of
         calibration} and results in an error model that can be represented as the
         action of the seven-dimensional matrix Lie group, $\Sim(3)$, on subsets of
         the measurements returned by the \lidarNoSpace.
    %  By focusing on the point clouds generated by the sensors, we motivate the application of shape-preserving transformations\footnote{Called \textit{similarity
    %      transformations} in projective geometry.}, that is a rigid body
    %      transformation plus a scale factor, in the calibration process. 

     \item One may suspect that our proposed model is over parameterized. We therefore  mathematically prove that given four targets with appropriate orientations, the proposed model is well-constrained (i.e., only one unique answer exists). The proof provides a guideline for target placement, which is an oriented tetrahedron.
     
     
    %  \addd{Parameterization analysis of the proposed model and the baselines is
    %          provided. Additionally, we mathematically prove that given four targets
    %          with appropriate orientations, the proposed model is well-constrained
    %      (i.e., only one unique answer exists).}\add{The proof provides a guideline
    %      for target placement, which is an oriented tetrahedron.}

     % \item \addd{We propose different ways to parse points on a target to collections
     %         of points. Each collection of points corresponds to a set of
     %         calibration parameters. We further propose kernelizing the traditional
     %         point-to-plane (P2P) distance while calibrating a \sslidar to smooth
     %         discontinuity of different sets of calibration parameters.}

     \item We propose a globally convergent algorithm to determine the calibration parameters. It utilizes an alternating optimization technique to solve the
         calibration problem where the scaling parameter is determined by the
     bisection method and the rest of the parameters ($\SE(3)$) are formulated as a
     Quadratically Constrained Quadratic Problem (QCQP) where the Langrangian dual
     relaxation is used. The relaxed problem becomes a Semidefinite Program (SDP) and
     convex~\cite{tron2015inclusion, carlone2015lagrangian, olsson2008solving,
     briales2017convex}. Therefore, the problem can be solved globally and
     efficiently by off-the-shelf specialized solvers~\cite{grant2014cvx}.

     \item We provide a MATLAB-based simulator for intrinsic \lidar calibration and
        validation that allows one to study the effects of target placement and the
        effectiveness of various calibration methods.

     % \item We show in simulation that our method can calibrate equally well a
     %     spinning \lidar and a \sslidarN. In experiments on a spinning \lidarNoSpace,
     %     we show that it works as well or better than two physics-based models. 
     \item In simulation, we validate that positioning the four
         targets as a tetrahedron can calibrate equally well a
         spinning \lidar and a \sslidarN. In experiments on a spinning \lidarNoSpace,
         we show that the proposed method works as well as two physics-based models in terms of P2P distance, while it is more robust when we induce systematic errors to the experimental measurements.
    
     \item We open-source all of the related software for intrinsic
        calibration, including implementations of the baseline methods, the simulator and the solver; see~\cite{githubFileIntrinsic, githubFileLiDARSimulator}\bh{add solver}. 

\end{enumerate}

% \mgj{Chenxi and Madhav did a good literature review. Let's shrink the introduction and add a Related Work section to make the paper more standard.}
% \href{https://www.overleaf.com/6951337515mwtqxhsjpyjk
% }{https://www.overleaf.com/6951337515mwtqxhsjpyjk
% }

%%\jwg{Talk about how this new model gives better results on actual data. To be written later.}

% This new calibration model has more expressivity than the three-parameter models in
% \cite{???}, and has equal expressivity and fewer parameters than the ten-parameter
% model in \cite{???}. With fewer parameters, the numerical convergence is better.
% \jwg{Stronger later???}


 %trim={<left> <lower> <right> <upper>}


==> JWG_Proof_Fragments.tex <==

   
   

==> Optimization_old.tex <==
\input{ExperimentTables}

\section{Global Optimization: from Min to Min-Min}
\label{sec:ConvexRelaxation}
Theorem~\ref{thm:uniqueness} states that a unique answer exists. In this section, we
propose a method to find it. In particular, we show a
globally convergent algorithm to determine the element of the Lie Group that globally
minimizes the cost function~\eqref{eq:P2PDistance}. This is done by converting the minimization
problem in~\eqref{eq:OptSolution} to a Min-Min problem. The inner minimization problem has an efficient global solution by results in~\cite{olsson2008solving, briales2017convex}. The outer minimization is scalar, and it is easy to limit the range of interest to a compact set. 

% \bh{compact subset of T and s, proposition}
\subsection{Problem Statement and Compact Sets}
\label{sec:CompactSets}
The intrinsic calibration problem is defined in~\eqref{eq:OptSolution}:
\begin{align}
    \label{eq:minOverSim}
    \min_{s,\R,\v}J(s,\R,\v; \Xcal_t, \n[t],\p[0,t]),
\end{align}
where $J$ is defined as
\begin{equation}
    \label{eq:P2PDistance2}
   \sum_{t=1}^T\sum_{i=1}^{M_t}
    \lvert \n[t][\transpose] \left( s\R \cdot \x[i] +\v- \p[0,t] \right) \rvert^2.
\end{equation}
Due to the unbounded $s\in\reals^+(\reals > 0)$ and $\v\in\reals^3$, we
consider a compact subset of $\v$ and $s$ so that there exists a solution ($J^\ast$)
to \eqref{eq:minOverSim}:
\begin{equation}
    J^\ast = \min_{s,\R,\v} J(s,\R,\v).
\end{equation}




% \begin{itemize}
%     \item define true problem
%     \item note SIM(3) is a product
%     \item  Fix s in R+ and define f(s) = min over SE(3) of the cost function
%     \item Then argue that $min_{R+} f(s) = min_{Sim(3) }$
% \end{itemize}
\input{SolverAlg}

\subsection{From Min to Min-Min}
\label{sec:MinMin}
$\Sim(3)$ can be written as a semi-direct product of the subgroups
$\reals^+$ and $\SE(3)$. We will use the fact that as a set, $\Sim(3)$ is
the Cartesian product of $\SE(3)$ and $\reals^+$, to redefine \eqref{eq:minOverSim}
as a \mm problem.
\begin{proposition}
\label{prop:MinToMinmin}
\begin{equation}
    \label{eq:MinEqualMinmin}
    \min_{s,\R,\v} J(s,\R,\v) = \min_s\min_{\R,\v}J(s,\R,\v)
\end{equation}
\end{proposition}
\textbf{Proof:} 
% We will prove the left-hand side and the right-hand side of
% \eqref{eq:MinEqualMinmin} is equal. 
In Sec.~\ref{sec:CompactSets}, we assume compact
subsets of $s$ and $\v$. Therefore, $\exists s^\ast, R^\ast, t^\ast$ such that
\begin{equation}
    J^\ast = J(s^\ast, R^\ast, t^\ast).
\end{equation}
We further define $h(s)$ as
\begin{equation}
h(s) := \inf_{\R,\v}J(s,\R,\v).
\end{equation}
Due to the existent of $J^\ast$, $\exists h^\ast$ such that
\begin{equation}
    h^\ast = \inf_s h(s) \implies h^\ast \le h(s), \forall s.
\end{equation}
By definition, we have
\begin{equation}
    \label{eq:JF}
    J^\ast \le h^\ast.
\end{equation}
To show $h^\ast \le J^\ast$, we consider 
\begin{equation}
    \label{eq:FJ}
h^\ast \le h(s^\ast) := {\inf_{\R,\v}J(s^\ast, \R,\v)} \le J(s^\ast, R^\ast, t^\ast) = J^\ast.
\end{equation}
\eqref{eq:JF} and \eqref{eq:FJ} concludes the equivalency of \eqref{eq:MinEqualMinmin}.\\
\qed


From Proposition~\ref{prop:MinToMinmin}, we can define the intrinsic calibration
problem as:
\begin{align}
    \label{eq:minS}
    f(s) = \min_{s}J(s;\R,\v,\Xcal_t, \n[t],\p[0,t]).
\end{align}




\comment{
\begin{itemize}
    \item $J^\ast=\min_{s,\R,\v}J(s,\R,\v) \implies \exists s^\ast, R^\ast, t^\ast$ such that $$ J^\ast = J(s^\ast, R^\ast, t^\ast)$$ 
    \item $f(s) := {\rm inf}_{\R,\v}J(s, \R,\v)$
    \item $f^\ast={\rm inf}_{s}f(s) \implies f^\ast \le f(s)$ for all $s$
    \item By definition, $J^\ast \le f^\ast $
\item  To show: $f^\ast \le J^\ast$. Consider 
$$f^\ast \le f(s^\ast) := {\inf_{\R,\v}J(s^\ast, \R,\v)} \le J(s^\ast, R^\ast, t^\ast) = J^\ast$$
\end{itemize}


Due to the property of the Cartesian product, given a scaling
$s\in\reals^+$, \eqref{eq:minOverSim} can be written as
\begin{align}
    \label{eq:minS}
    f(s) = \min_{\R,\v}J(\R,\v;s,\Xcal_t, \n[t],\p[0,t]),
\end{align}
which has an efficient global solution~\cite{olsson2008solving, briales2017convex}.
Therefore, \eqref{eq:minOverSim} is a \mm problem:
\begin{equation}
    \label{eq:minmin}
    \min_{s}\min_{\R,\v}\sum_{t=1}^T J_t(s,\R,\v; \Xcal_t, \n[t],\p[0,t]).
\end{equation}
\begin{itemize}
    \item $J^\ast=\min_{s,\R,\v}J(s,\R,\v) \implies \exists s^\ast, R^\ast, t^\ast$ such that $$ J^\ast = J(s^\ast, R^\ast, t^\ast)$$ 
    \item $f(s) := {\rm inf}_{\R,\v}J(s, \R,\v)$
    \item $f^\ast={\rm inf}_{s}f(s) \implies f^\ast \le f(s)$ for all $s$
    \item By definition, $J^\ast \le f^\ast $
\item  To show: $f^\ast \le J^\ast$. Consider 
$$f^\ast \le f(s^\ast) := {\inf_{\R,\v}J(s^\ast, \R,\v)} \le J(s^\ast, R^\ast, t^\ast) = J^\ast$$
\end{itemize}
}

\add{
\begin{remark}
    If we have one unique answer to Problem~\ref{prob:intrinsic_calibration} (states in
    Theorem~\ref{thm:uniqueness} and Sec.~\ref{sec:CompactSets}), we strongly
    conjecture that \eqref{eq:minS} is convex, because all of our
    datasets and the datasets from~\cite{olsson2008solving, briales2017convex} show
    the convexity, as shown in Fig.~\ref{fig:Solver}. The proof is still an ongoing
work. 
\end{remark}
}
% Being able to have one unique answer to Problem~\ref{prob:intrinsic_calibration}
% is critical (states in Theorem~\ref{thm:uniqueness}). Without the uniqueness
% constraint,~\eqref{eq:minS} is not convex, see
% Appendix~\ref{sec:DualFormulation}. 

\subsection{Parameter of Scaling Determination}
\addd{
Theoretically, a dense search on the scaling $s$ should be performed on a range of
interest. However, we empirically observed that \eqref{eq:minS} is always convex, see 
Sec.~\ref{sec:MinMin}. We, therefore, utilize the bisection method to determine
the scaling $s$. The proof of the convexity is an ongoing work.
}
% Theoretically, a dense search on the scaling $s$ should be performed on a range of
% interest. However, we empirically show that \eqref{eq:minS} is always convex, see 
% Sec.~\ref{sec:MinMin}. We, therefore, utilize the bisection method to determine
% the scaling $s$.


\addd{
    Let $\pre[k][L]s$ and $\pre[k][U]s$ be the lower and upper bounds
    of the scaling parameters at the $k$-th iteration. Let $\pre[k+1]s^\prime =
    (\pre[k][U]s + \pre[k][L]s)/2$ be the update for $(k+1)$-th iteration. The
    updates of the scaling parameters are defined as:
\begin{align}
    \label{eq:UpdateScaling}
    \pre[k+1][L]s &=
\begin{cases}
    s^\prime, \text{~if~}f(\pre[k][U]s)<f(\pre[k][L]s) \\
\pre[k][L]s, \text{~~~~~~otherwise}
\end{cases}\nonumber\\
    \pre[k+1][U]s &=
\begin{cases}
    s^\prime, \text{~if~}f(\pre[k][L]s)<f(\pre[k][U]s) \\
\pre[k][U]s, \text{~~~~~~otherwise}
\end{cases}.
\end{align}
}
\begin{figure}[b]%
\centering
\includegraphics[width=0.9\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{convexity2.png}%
\caption[]{\add{This figure illustrates \eqref{eq:minS} is potential convex and the
        proof is an ongoing work. If \eqref{eq:minS} is indeed proven as convex, then
        the bisection method can be performed instead of the dense search to find the
        global optimum.}}
\label{fig:Solver}
\end{figure}
% \begin{figure}[b]%
% \centering
% \subfloat{%
% \label{fig:SolverExpSetup}%
% \includegraphics[height=0.15\textheight, trim={0cm 0cm 0cm 0cm},clip]{FSconvex.png}}%
% \hspace{2pt}
% \subfloat{%
% \label{fig:SolverResults}%
% \includegraphics[height=0.15\textheight, trim={2cm 0cm 0cm 0cm},clip]{placeholder.png}}
% \caption[]{\bhp{For the solver}}
% \label{fig:Solver}
% \end{figure}
\addd{
At the $(k+1)$-th iteration, the scaling parameter is determined and the rest of the
parameters are $\SE(3)$. To solve the remaining parameters, we adopt techniques that
were used to solve 3D registration or 3D SLAM~\cite{tron2015inclusion,
carlone2015lagrangian, olsson2008solving, briales2017convex} where the problem is
formulated as a QCQP, and the Lagrangian dual relaxation is used. The relaxed
problem becomes a Semidefinite Program (SDP) and convex. The problem
can thus be solved globally and efficiently by off-the-shelf specialized
solvers~\cite{grant2014cvx}. This process is summarized in
Appendix~\ref{sec:DualFormulation}. As shown in~\cite{briales2017convex} the dual
relaxation is empirically always tight (the duality gap is zero). We also use the
same simulation and experimental dataset in~\cite{olsson2008solving,
briales2017convex} to verify that the proposed algorithm is able to converge
globally, see Appendix~\ref{sec:DualFormulation} for more visual results.
}




==> PlaneEstimation.tex <==
\section{Plane Estimation}
\label{sec:lidarVertices}
\addd{Indicated in Sec.~\ref{sec:IntrinsicCalibration}, the normal vector of a target
(i.e. the plane equation), must be estimated from data. Due to the assumption that the
wafer of an OPA \sslidar is slightly warped (see Sec.~\ref{sec:ExpSSLiDAR}),
directly estimating the plane equation using existing methods in the literature is
inviable because they do not take this geometric distortion into account. This
section therefore provides two means to estimate the normal vectors from a \slidar
and \sslidar.}

\subsection{Plane Estimation for \slidars}
\addd{The following is partially taken from \cite{huang2020improvements} and provided for
clarity.
Let $\pc := \{\calx_i\}_{i=1}^{M}$ be a collection of 3D points on a \lidar target,
where $M$ is the number of points. Given the target geometry, we define an ideal
target with vertices $\{ \bar{X}_i \}_{i=1}^4$ located at the origin of the \lidarN.
% as defined in Fig.~\ref{fig:IdealFrame}.
We seek a rigid body transformation from \lidar to the target, $H_L^T$, that ``best
fits'' the ideal target onto the point cloud.}

\addd{In practice, it is actually easier to pull the $\pc$ back to the origin of the LiDAR
through the inverse of the current estimate of transformation $H_T^L:=(H_L^T)^{-1}$
and measure the error there. For $a \ge 0$ and $\lambda \in \real^+$, an
$L_1$-inspired cost is defined as
\begin{equation}
    \label{eq:L1cost}
    c(\lambda,a):=\begin{cases}
    \min\{ |\lambda-a|, |\lambda + a| \} & \text{if}~|\lambda| >a \\
    0 & \text{otherwise}
    \end{cases}.
\end{equation}
Let $\{\tilde{\calx}_i\}_{i=1}^N:=H_T^L(\mathcal{PC}):=\{ H_T^L(\calx_i) \}_{i=1}^N$ denote
the pullback of the point cloud by $H_T^L$, and denote a point's $(x,y,z)$-entries by
$(\tilde{x}_i,\tilde{y}_i,\tilde{z}_i)$.
The total fitting error of the point cloud is defined as
\begin{equation}
	\label{eq:JKHcost}
    C(H_T^L(\pc)) :=\sum_{i=1}^{M} c(\tilde{x}_i,\epsilon) +
    c(\tilde{y}_i,d/2) +  c(\tilde{z}_i,d/2),
\end{equation}
where $\epsilon \ge 0$ is a parameter (estimated by the smallest variance of the
principal axis), to account for uncertainty in the depth
measurement of the planar target. For more detail about this method and target
placement for extrinsic calibration, see~\cite{huang2020improvements}. Once we
estimate the four vertices of the target, the plane equation of the target is
trivial. The estimated plane is shown in Fig.~\ref{fig:L1PlaneEstimation}.}


\subsection{Plane Estimation for \sslidars}
\addd{Due to the warped wafer, the closer to the edge of the wafer, the larger the
distortion is. We therefore estimate the target's normal vector by weighted least squares
where the weight is the distance of each point to the mean of all the points on the
target. Figure~\ref{fig:WeightedPlaneEstimation} shows the result of plane estimation
against the ground truth from the simulator.}

\begin{figure}[b]%
\centering
\subfloat{%
    \label{fig:L1PlaneEstimation}%
\includegraphics[width=0.48\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{placeholder.png}}~
\subfloat{%
    \label{fig:WeightedPlaneEstimation}%
\includegraphics[width=0.48\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{placeholder.png}}
\caption[]{\bhp{}}
\end{figure}


% \textbf{Calibration Method:} Let ${\cal PC}$ be a union of point clouds for
% a collection of planar targets, and separate the points by ring number, giving $K$
% point clouds, ${\cal PC}_k$, $1 \le k \le K$. For the $k$-th point cloud, determine a
% best collection of calibration parameters  $\alpha^*_k$ from \eqref{eq:OptSolution}. The collection of
% calibartion determines a calibration for the \lidar. The calibrated points are
% \bh{blah blah blah}

% \begin{remark}
% The decomposition of the point cloud by rings is motivated by a
% spinning \lidar. For a \lidar such as ????, one might decompose the point cloud
% as ????
% \end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> PreJessyAutomaticCalibrationPipeline.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Automatic Calibration System}
\label{sec:AutomaticCalibrationSystem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Target-based \lc extrinsic calibration methods often suffer from manual target
extraction and feature association. In our previous
work~\cite{huang2019improvements} that addressed the estimation of  \lidar target vertices and extrinsic
calibration, we assumed \lidar points falling on the target were extracted by hand and the camera corners were obtained manually by clicking on an image. Because experimentally comparing and validating the intrinsic calibration methods of
Sec.~\ref{sec:IntrinsicCalibration} and~\ref{sec:Baseline} would require significant
data collection, we decided to create a fully automatic pipeline for both intrinsic
and extrinsic calibration, as shown in Fig~\ref{fig:AutomaticPipeline}. We demonstrate the capability of this
pipeline by collecting a significant amount of data allowing us to check the quality
of the calibration of our sensor suite (a \lc pair) at different distances;
see~\ref{sec:EXPExtrinsicCalibration}.

% The front-end of the pipeline includes data acquisition, sensor synchronization,
% \lidar and camera targets extraction, as well as target association. The back-end
% extracts vertices of the \lidar targets, vertex-corner association, and extrinsic
% calibration. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.3\columnwidth]{graphics/AutomaticPipeline.png}
    \caption{\bh{add intrinsic calibration to the system diagram}A system diagram for
        automatic intrinsic and extrinsic calibration. The top shows the front-end of
        the pipeline. Its input is raw camera and \lidar data, which are subsequently
        synchronized. The \atag and \lidart packages are used to extract the target
        information, which is then examined to remove outliers and ensure that
        targets are still properly synchronized. Each run of the front-end saves all
        related information into a ROS bagfile, which can then be sent to the
        back-end for further processing. The back-end takes in (possibly many) ROS
        bagfiles and does the following: (i) refines the image corners; and (ii)
        extracts vertices of the \lidar targets. The correspondences are established
        between corners and vertices and an extrinsic transformation is determined
        PnP as in \cite{lepetit2009epnp}. For intrinsic calibration, the resulting vertices of
        the \lidar targets are used to extract normal vectors and a point on the
        plane. The calibration parameters are determined to minimize the P2P distance
        from the plane to the target points provided by the \lidart package.} 
\label{fig:AutomaticPipeline}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Front-End: Data Pre-processing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The first step in target-based calibration is to estimate independent target features from
% a \lidar point cloud and a camera image. In this paper, we use target vertices as our
% features. 

Fiducial markers, such \atagsN\cite{olson2011apriltag, wang2016apriltag,
krogiusflexible}, are widely used in vision-based perception tasks because they can
be  easily identified and automatically extracted from background. In
\cite{huang2019lidartag}, we introduced a similar concept for \lidar point clouds,
called a \lidartN.  Inspired by \atags, they consist of a payload and a pattern that
makes each marker uniquely distinguishable and identifiable in real-time by both a
\lidar and a camera. An open-source package for processing \lidarts is available
\cite{githubFileLiDARTag}, while \atagN3 is available as a ROS package
\cite{githubFileAprilTagROS}. 

As the \lidar and camera data streams arrive, they are synchronized, examined for
fiducial markers, and checked for false positives. For \lc extrinsic calibration,
corresponding features from camera data and \lidar data must be identified. We use
target vertices as our features in this pipeline. In the image plane, the target
vertices are typically called corners and are extracted in the front end using the
\atag ROS package. The relevant information is saved as ROS bagfiles so that they can
be loaded directly into MATLAB for post-processing. The technical details and
the software are available on Github\cite{githubFileAutoCalibration}.

% Fiducial markers are widely used in navigation as well as vision-based simultaneous
% localization and mapping (SLAM). They often consist of a payload, a pattern that
% makes each marker uniquely distinguishable. Therefore, as an aid in the automatic
% identification of targets, we build and use fiducial markers that can be identified
% by both a \lidar and a camera. To extract fiducial markers from an image, \atag
% package is typically used; similarly for \lidar point cloud, we develop a type of
% fiducial marker that can be detected in real-time from \lidar point clouds:
% \lidartN~\bh{cite}. Due to false positive from detection algorithms, further
% examination (outliers removal) of the extracted features is crucial. Because image
% are raw measurement (i.e., they will not be missing), we ensure the indices of the
% two types of detection are the same as the image's index before publishing. All the
% related information are saved as ROS bagfiles and will be loaded directly from
% MATLAB. For more technical detail about each step, see our Github\bh{gitbub}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Back-End: Data Post-processing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
At this stage, extracted features (\atag corners and \lidart points) have been
properly synchronized and examined automatically for false positives. The next step
is to estimate the \lidart vertices, which, due to sparsity of the \lidar point
cloud, are not directly observable. We use the method developed in
\cite{huang2019improvements} to determine the vertices of a diamond-shaped target.
From the vertices, the target normal $\n[t]$ and point on the target, $\p[0,t]$, can
be easily determined for evaluating the P2P cost function
\eqref{eq:OptSolution} for intrinsic calibration, while the vertices in
combination with the camera corners are used to
determine the extrinsic calibration via a PnP problem.
 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\columnwidth, trim={0.05cm 0cm 0cm 1cm},clip] {graphics/reference_frame2.png}
%     \caption{\bh{Notation}Target reference frame and real point cloud data.
%         The dotted blue square is the reference target; its vertices are denoted
%         $\{\bar{X}_i\}_{i=1}^4$.} 
% \label{fig:IdealFrame}
% \end{figure}

\begin{figure}[t]%
\centering
\subfloat[]{%
\label{fig:IdealFrame}%
\includegraphics[width=0.45\columnwidth, trim={0.05cm 0cm 0cm 1cm},clip] {graphics/reference_frame2.png}}~
\subfloat[]{%
\label{fig:CannyLineFitted}%
\includegraphics[width=0.48\columnwidth, trim={3.5cm 12.6cm 3cm 10cm},clip]{CannyLineFitted.png}}\\
\subfloat[]{%
\label{fig:CalibrationResults}%
\includegraphics[width=0.45\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test6_3.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:CannyLineFitted}%
\includegraphics[width=0.5\columnwidth, trim={2cm 1.7cm 2cm 0.7cm},clip]{test6_3.png}}
\caption[]{\bh{Notation, not much space, may remove
later}\subref{fig:IdealFrame}Target reference frame and real point cloud data.
The dotted blue square is the reference target; its vertices are denoted
$\{\bar{X}_i\}_{i=1}^4$.\subref{fig:CannyLineFitted} shows the result of edge
detection. }% 
\label{fig:ImageEdgeDetection}%
\squeezeup
\end{figure}


\subsubsection{Finding \lidar vertices}
\label{sec:lidarVertices}
The following is taken from \cite{huang2019improvements} and provided for clarity. \jwg{Check consistency of our notation for points in a PC.}\bh{currently, I leave math notation as it is. I will closely read our notation and then fix them altogether.}
Let $\pc := \{\calx_i\}_{i=1}^{M}$ be a collection of 3D points on a \lidar target,
where $M$ is the number of points. Given the target geometry, we define an ideal
target with vertices $\{ \bar{X}_i \}_{i=1}^4$ located at the origin of the \lidar as
defined in Fig.~\ref{fig:IdealFrame}. We seek a rigid body transformation from \lidar
to the target, $H_L^T$, that ``best fits'' the ideal target onto the point cloud. 

In practice, it is actually
easier to pull the $\pc$ back to the origin of the LiDAR through the inverse of the
current estimate of transformation $H_T^L:=(H_L^T)^{-1}$ and measure the error there. 
For $a \ge 0$ and $\lambda \in \real^+$, an $L_1$-inspired cost
is defined as 
\begin{equation}
    \label{eq:L1cost}
    c(\lambda,a):=\begin{cases} 
    \min\{ |\lambda-a|, |\lambda + a| \} & \text{if}~|\lambda| >a \\
    0 & \text{otherwise}
    \end{cases}.
\end{equation}
Let $\{\tilde{\chi}_i\}_{i=1}^N:=H_T^L(\mathcal{PC}):=\{ H_T^L(\chi_i) \}_{i=1}^N$ denote
the pullback of the point cloud by $H_T^L$, and denote a point's $(x,y,z)$-entries by
$(\tilde{x}_i,\tilde{y}_i,\tilde{z}_i)$.
The total fitting error of the point cloud is defined as 
\begin{equation}
	\label{eq:JKHcost}
    C(H_T^L(\pc)) :=\sum_{i=1}^{M} c(\tilde{x}_i,\epsilon) +
    c(\tilde{y}_i,d/2) +  c(\tilde{z}_i,d/2),
\end{equation}
where $\epsilon \ge 0$ is a tuning parameter to account for uncertainty in the depth
measurement of the planar target. For more detail about this method and target
placement for extrinsic calibration, see~\cite{huang2019improvements}.


\subsubsection{Corner Extraction and Association with Vertices}
The only manual process in our previous software release, determining the image corners, has now
been made automatic. The corners obtained from the \atag package are automatically
refined as shown in Fig.~\ref{fig:CannyLineFitted} using a process detailed in
\cite{huang2019improvements}. Given the camera corners ($\{ Y_i\}_{i=1}^4$) and \lidar vertices
$\{ X_i\}_{i=1}^4$, we use the vertical and horizontal positions in their own
coordinates to sort them and establish the correspondences.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Intrinsic and Extrinsic Calibration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:InExCalibration}
For extrinsic calibration, once ``enough'' independent target vertices are estimated
from both camera data and \lidar point cloud, the \lidar to camera extrinsic
transformation is solved by Perspective-n-Point (PnP) as in \cite{lepetit2009epnp},
\begin{equation} 
    \label{eq:ConceptualProblem} (R_{C}^{L*}, T_{C}^{L*})= \mathrm{arg}
    \min_{(R,T)}{\mathrm{dist}(P(H_{L}^{C}(X_i)),Y_i)}, 
\end{equation} 
where $X_i$ are the (homogeneous) coordinates of the \lidar features, $Y_i$ are the
coordinates of the camera features, $P$ is the often-called `projection map'',
$H_{L}^{C}$ is the \lidarN-frame to camera-frame transformation with rotation matrix
$R_{C}^{L}$ and translation $T_{C}^{L}$, and $\mathrm{dist}$ is a distance or error
measure. An example of extrinsic calibration is shown in
Fig.~\ref{fig:CalibrationResults}. More detail is provided
in~\cite{huang2019improvements}.

For intrinsic calibration, the target vertices are used to compute a normal vector and a
point on the target. The P2P distance is minimized for each of the three calibration
models, \BL1, \BL2, and $\Sim(3)$, for a collection of targets, yielding $\alpha^*$
(for \BL1 and \BL2) and  $\Sigma^*$ for $\Sim(3)$.

The processes of intrinsic calibration involves iterating the estimation of the
target vertices and the parameters in the \lidar model until a given stopping
criterion is met. Here, we stopped when the maximum change $\delta_m$ over the set of target vertices was less
than $1e-5$.

\begin{algorithmic}
\While{$\delta_m>1e^{-5}$} 
\State \textbf{Step 1:} Re-estimate the target vertices $\{ X_i\}_{i=1}^4$
after applying the  current intrinsic calibration parameters to the point
cloud. This gives updated values for the target normals and points on the
targets.
\State \noindent \textbf{Step 2:} Using the updated target vertices, re-estimate the
intrinsic calibration parameters for the three calibration models.

\EndWhile
\end{algorithmic}
% \noindent \textbf{DO UNTIL} \jwg{algorithm environment?}\\
% \noindent \textbf{Step 1:} Re-estimate the target vertices $\{ X_i\}_{i=1}^4$ after applying the  current intrinsic calibration parameters to the point cloud. This gives updated values for the target normals and points on the targets.
% 
% \noindent \textbf{Step 2:} Using the updated target vertices, re-estimate the intrinsic calibration parameters for the three calibration models.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\subsection{System Overview}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \subsection{Sensor Synchronization and Feature Extraction}
% Due to the \lidar and camera data arriving at different rates, they have to be
% properly synchronized, especially, if the calibration scene is not static. Because
% the camera frames are roughly at 30 Hz and \lidar packets are at 10 Hz, the
% \textit{ApproximateTime} policy in Robot Operating System (ROS) can be used for
% synchronization ~\cite{quigley2009ros}. The synchronized data 
% are indexed and sent to appropriate packages for feature extraction.
% 
% Fiducial markers are widely used in navigation as well as
% vision-based simultaneous localization and mapping (SLAM). They often consist
% of a payload, a pattern that makes each marker uniquely distinguishable.
% Therefore, as an aid in the automatic identification of targets in
% camera and \lidar data, we build and use fiducial markers that can be identified by
% both a \lidar and a camera.  
% 
% 
% \subsubsection{camera targets}
% Images containing calibration targets are processed using the latest \atag3
% package~\bh{cite \atag1, \atag2, \atag3, Github}. The package is written in C++
% on the ROS platform and provides the (inner) corners of the fiducail marker and the
% corresponding ID. The target vertices, however, are the outer corners as shown in
% Fig~\bh{InnerOuterCorners}. Given the homography matrix and the intrinsic parameters of the
% camera, the outer corners can be determined with simple linear interpolation.
% For more detail, see~\bh{\atag1}
% 
% 
% \subsubsection{\lidar targets}
% Point clouds containing the calibration targets are sent to \lidart
% package\bh{cite}. \lidart is a type of fiducial marker that can be detected
% n real-time from \lidar point clouds, called \lidartsN.
% The released
% version of \lidart provides the points on the target and tag size associated with the target. The
% target points are then post-processed by an $L_1$-inspired norm to determine the vertices;
% see~\ref{sec:LiDARVertices} and \bh{cite}.
% 
% \begin{remark}
% don't care poses
% \end{remark}
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Target Association}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Due to false positive from detection algorithms, further examination of the extracted
% features is crucial. As mentioned, we have indexed the synchronized data and they are
% used as a tracking id. We have three messages to associate: images, \atags and
% \lidartsN. Each of them has its own queue and because images are raw measurement, we
% ensure the indices of the two types of detection are the same as the image's index,
% before publishing. We also create a global sequence queue to track the
% candidate index to publish. ~\bh{working on...}
% 
% % Whenever a new message arrives, the frame index of this message will pushed to
% % its own queue and the global sequence queue if it is in order. 
% % When the front of three message queues have the same frame index, we shall group them
% % together and publish.
% % 
% % Lastly, the detection messages with the same index are grouped as a new paired message. 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Finding LiDAR Corners and Corners Association}
% \label{sec:LiDARVertices}
% \label{sec:CornerAssociation}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% At this stage, extracted features (\atag corners and \lidart points) have been
% properly synchronized and cautiously examined. An $L_1$-inspired norm is applied to
% estimate non-directly observable \lidart vertices. Given Let $\pc := \{X_i\}_{i=1}^{M}$
% be the collection of 3D points on the \lidar target, where $M$ is the number of
% points. For $a \ge 0$ and $\lambda \in \real$, the $L_1$-inspired cost is defined as 
% \begin{equation}
%     \label{eq:L1cost}
%     c(\lambda,a):=\begin{cases} 
%     \min\{ |\lambda-a|, |\lambda + a| \} & \text{if}~|\lambda| >a \\
%     0 & \text{otherwise}
%     \end{cases},
% \end{equation}
% and the total cost is define as 
% \begin{equation}
% 	\label{eq:JKHcost}
%     C(H_T^L(\pc)) :=\sum_{i=1}^{M} c(\tilde{x}_i,\epsilon) +
%     c(\tilde{y}_i,d/2) +  c(\tilde{z}_i,d/2),
% \end{equation}
% where $\epsilon \ge 0$ is a tuning parameter to account for uncertainty in the depth
% measurement of the planar target. For more detail about this method and target
% placement for extrinsic calibration, see~\bh{cite}.
% 
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Extrinsic Calibration}
% \label{sec:ExtrinsicCalibration}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Related.tex <==
\section{Related Work}
\label{sec:related_work}

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bruce.png}}]{Jiunn-Kai Huang} received the Master's degree in robotics from the University of Michigan, Ann Arbor in 2018.  He is currently a Ph.D. candidate in robotics at the University of Michigan, Ann Arbor. His current research interests are perception, sensor fusion and motion planning. He has also researched perception for action recognition and 3D skeleton pose estimation to assist autonomous vehicles in navigating near humans.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,trim={0cm 15cm 0cm 14cm},clip,keepaspectratio]{Chenxi.jpeg}}]{Chenxi Feng} received the Master's degree in Mechanical Engineering from the University of Michigan, Ann Arbor in 2020. His research interests are sensor calibration and multi-sensor fusion. He is currently working on high definition map for autonomous vehicles at Nvidia.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{madhav.png}}]{Madhav Achar} graduated from the University of Michigan with a bachelors in computer engineering and a Masters in Robotics. He has previously worked as a software engineer at Bosch working in their perception team. Currently he works at Quantum Signal AI tackling problems in planning, controls and simulation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{maani_ghaffari.jpg}}]{Maani Ghaffari}
received the Ph.D. degree from the Centre for Autonomous Systems (CAS), University of Technology Sydney, NSW, Australia, in 2017. He is currently an Assistant Professor at the Robotics Institute and Department of Naval Architecture and Marine Engineering, University of Michigan, Ann Arbor, MI, USA. He recently established the Computational Autonomy and Robotics Laboratory. His research interests lie in the theory and applications of robotics and autonomous systems.
\end{IEEEbiography}





\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{headshotJWG2.jpg}}]{Jessy W. Grizzle} (S’78–M’83–F’97) received the Ph.D. in electrical engineering from The University of Texas at Austin in 1983. He is the Director of the Michigan Robotics Institute and a Professor of Electrical Engineering and Computer Science at the University of Michigan, where he holds the titles of the Elmer Gilbert Distinguished University Professor and the Jerry and Carol Levin Professor of Engineering. He jointly holds sixteen patents dealing with emissions reduction in passenger vehicles through improved control system design. Professor Grizzle is a Fellow of the IEEE and IFAC. He received the Paper of the Year Award from the IEEE Vehicular Technology Society in 1993, the George S. Axelby Award in 2002, the Control Systems Technology Award in 2003, the Bode Prize in 2012, the IEEE Transactions on Control Systems Technology Outstanding Paper Award in 2014, and the  IEEE Transactions on Automation Science and Engineering, Googol Best New Application Paper Award in 2019. His work on bipedal locomotion has been the object of numerous plenary lectures and has been featured on CNN, ESPN, Discovery Channel, The Economist, Wired Magazine, Discover Magazine, Scientific American and Popular Mechanics.
\end{IEEEbiography}

==> defines_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% normal packages
\usepackage{bmpsize}
\usepackage{amsthm}
\usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage{amsmath,amssymb,enumerate}
\usepackage{mathrsfs}
\usepackage{times}
\usepackage{multicol}
\usepackage{amsfonts}
\usepackage{textcomp}
\usepackage{balance}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{dblfloatfix} 

\usepackage{bbold}
\usepackage{makecell}
\usepackage{hhline} % double-line in a table

\usepackage{comment}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{soul} 
\usepackage{times}
% \usepackage{fixltx2e}
\usepackage{balance}
% \usepackage{graphicx}


% packages with options
\usepackage[dvipdfmx]{graphicx} 
\usepackage[T1]{fontenc}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage[utf8]{inputenc}
% \usepackage[title]{appendix}


% packages with setups
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed
}

\usepackage{caption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}
% \let\proof\relax 
% \let\endproof\relax



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Graphics path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\graphicspath{
    {graphics/}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {\itshape}{}%
  {\bfseries}{}%
  {\newline}{}%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\theoremstyle{break}
% \newcounter{exercises}
\newtheorem{assumption}{Assumption}
% \setcounter{assumption}{0}

% \newtheorem{claim}[theorem]{Claim}
\newtheorem{claim}{Claim}

% proof style
\renewcommand\qedsymbol{$\blacksquare$}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm inputs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\rha}[1]{[{\textbf{\textcolor{orange}{Ross: #1}}}]}
\newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{teal}{Maani: #1}}}]}
\newcommand{\jkh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bht}[1]{[{\textbf{\textcolor{note}{Bruce: (TODO) #1}}}]}
\newcommand{\bhw}[1]{[{\textbf{\textcolor{note}{Bruce: working in progress #1}}}]}
\newcommand{\bhd}[1]{[{\textbf{\textcolor{blue}{Bruce: Done, please check#1}}}]}
\definecolor{note}{rgb}{0.3,0.7,0.25}
\definecolor{rephase}{rgb}{0.15,0.7,0.15}
\definecolor{bag}{rgb}{0.6,0.6,0.2}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lc}{LiDAR-camera~}
\newcommand{\LC}{LiDAR-Camera~}
\newcommand{\lidar}{LiDAR~}
\newcommand{\lidarNoSpace}{LiDAR}
\newcommand{\lidarN}{LiDAR}
\newcommand{\lidars}{LiDARs~}
\newcommand{\lidarsN}{LiDARs}
\newcommand{\velodyne}{\textit{32-Beam Velodyne ULTRA Puck LiDAR~}}
\newcommand{\velodyneN}{\textit{32-Beam Velodyne ULTRA Puck LiDAR}}

\newcommand{\sslidar}{solid-state LiDAR~}
\newcommand{\sslidarN}{solid-state LiDAR}
\newcommand{\sslidars}{solid-state LiDARs~}
\newcommand{\sslidarsN}{solid-state LiDARs}

\newcommand{\slidar}{spinning LiDAR~}
\newcommand{\slidarN}{spinning LiDAR}
\newcommand{\slidars}{spinning LiDARs~}
\newcommand{\slidarsN}{spinning LiDARs}

\newcommand{\lidart}{LiDARTag~}
\newcommand{\lidarts}{LiDARTags~}
\newcommand{\lidartN}{LiDARTag}
\newcommand{\lidartsN}{LiDARTags}

\newcommand{\ltag}{LiDARTag~}
\newcommand{\ltagN}{LiDARTag}
\newcommand{\ltags}{LiDARTags~}
\newcommand{\ltagsN}{LiDARTags}

\newcommand{\atag}{AprilTag~}
\newcommand{\atags}{AprilTags~}
\newcommand{\atagN}{AprilTag}
\newcommand{\atagsN}{AprilTags}

\newcommand{\lind}{linearly independent}
\newcommand{\li}{linearly independent}
\newcommand{\ld}{linearly dependent}

\newcommand{\dom}{\mathrm{dom}}
\newcommand{\BL}{\textbf{BL}}
\newcommand{\bl}{\textbf{BL}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% functionalities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\squeezeup}{\vspace{-4mm}} % save space
% \long\def\/*#1*/{} % block comments: \/* */



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematics Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\realnumbers{\mathbb{R}}
\def\real{\mathbb{R}}
\def\reals{\mathbb{R}}

\newcommand{\pc}{\mathcal{PC}}
\newcommand{\GPcal}{\mathcal{GP}}
\newcommand{\calx}{\mathcal{X}}
\newcommand{\dtheta}{\delta_\theta}
\newcommand{\dphi}{\delta_\phi}
\newcommand{\drho}{\delta_\rho}
\newcommand{\ep}{\mathcal{EP}}
\newcommand{\Pring}{\mathcal{P}}
\newcommand{\vx}{\mathcal{V}}



% operations
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\transpose}{\mathsf{T}}
% \newcommand{\span}[1]{\left{#1\right}}


% Groups and Algebra
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\Sim}{\mathrm{Sim}}
\newcommand{\Exp}{\mathrm{Exp}}
% \newcommand{\Log}{\mathrm{Log}}
% \newcommand{\Jr}{\mathrm{J_r}}

% Trigonometry
\DeclareDocumentCommand{\asin}{ O{} }{\sin^{-1}(#1)}
\DeclareDocumentCommand{\acos}{ O{} }{\cos^{-1}(#1)}
\DeclareDocumentCommand{\atan}{ O{} }{\tan^{-1}(#1)}


\DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
\DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
\DeclareDocumentCommand{\pre}{ O{} O{} }{{}_{#1}^{#2}}


% \newcommand{\GL}{\mathrm{GL}}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance

% \newcommand{\diag}{\mathop{\mathrm{diag}}}
% \newcommand{\m}{\mathop{\mathrm{m}}}
% \newcommand{\rad}{\mathop{\mathrm{rad}}}
% \newcommand{\dBm}{\mathop{\mathrm{dBm}}}
% \newcommand{\Hz}{\mathop{\mathrm{Hz}}}
% \newcommand{\GHz}{\mathop{\mathrm{GHz}}}
% \newcommand{\MHz}{\mathop{\mathrm{MHz}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Cal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
% \newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
% \newcommand{\Fcal}{\mathcal{F}}
% \newcommand{\Hcal}{\mathcal{H}}
% \newcommand{\Ical}{\mathcal{I}}
% \newcommand{\Kcal}{\mathcal{K}}
% \newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Scal}{\mathcal{S}}
% \newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}
% \newcommand{\Ycal}{\mathcal{Y}}
% \newcommand{\Zcal}{\mathcal{Z}}


% lowers
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands for letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
\DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
\DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
\DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
\DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
\DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
\DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
\DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
% \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
\DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
\DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
\DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
\DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
\DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
\DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
% \DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}


% lowers
\DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
\DeclareDocumentCommand{\n}{ O{} O{} }{\textbf{n}_{#1}^{#2}}
\DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
\DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
\DeclareDocumentCommand{\q}{ O{} O{} }{\textbf{q}_{#1}^{#2}}
\DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
\DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
\DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other New commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}


% \makeatletter
% \newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
% \newcommand{\mathcenter}{\@fleqnfalse}
% \makeatother


==> notes.tex <==
\section*{Notes for ourselves}
Color code: \add{green} and \addd{brown} are the newly added sentences/
paragraphs. All of the automatic calibration related paragraphs are removed. 
The paper is too long now; I would suggest removing the plane estimation section. It
is still not enough (it would be around 8.6 pages). By reducing some white space and
shrinking some figures or shorten some paragraphs might fit to 8-page. 


Several points from the reviewers (I am still working on addressing them and
cross-out means the issue is addressed): 
\begin{enumerate}
\item More experiments with real data are needed. \bh{Shows some rings are
    poorly calibrated before and well-calibrated after.}
\item Provide more experimental validation from real data (both spinning lidar and
    solid state lidar). \bh{We don't have a solid state lidar yet but for spinning
    lidars, it could be the same as above.}
\item The computation time should be included.
\item How to get the initialization of the optimization problem? The authors should
    discuss the estimation of an initial solution, and how the error of an initial
    solution can impact on the convergence of the optimization algorithm.\bh{I will
    add this to experimental results.} 
\item Maybe add noise N1/N2 as described in the paper to the real data. \bh{This is
    actually a good idea.}
\item What is Table 3 reporting? \bh{Need to explain more}
\item What is the interest of this model? You claim that it is better than others,
    but what is your criterion ? How do you assess / prove it ? The experiments on
    simulated data only are weak.
\item What are the two type of uncertainities in Section V.A. \bh{Need to explain
    more}
\item Video: The presentation is good, but the image is deteriorated by
the compression and it is hard to read the captions.
Consider shortening the length of the video or using audio
for the conference video. \bh{Make the video shorter and larger captions}
\item \dels{What is the minimal case to determine the model parameters? How many
    solutions are there for the minimal case?}
\item \dels{The authors should focus only on the intrinsic calibration.}
\item \dels{How is error calculated in Table 1, what is the unit of
error?}
\item \dels{How is geometric uncertainty defined for Table 2?}
\item \dels{Table 3 shows the misleading results since the values in "Our Method" are in
    bold where the minimum value is originally in bold.}
\item \dels{It is interesting if the 7-parameters rigid body
transformation can approximate the intrinsic parameter.
However, the novelty looks week because the method just
replacing the model. Therefore, deeper evaluation and
discussion is required.}
\end{enumerate}
